A-FMI: Learning Attributions from Deep Networks via Feature Map Importance

Gradient-based attribution methods can aid in the understanding of convolutional neural networks (CNNs). However, the redundancy of attribution features and the gradient saturation problem, which weaken the ability to identify significant features and cause an explanation focus shift, are challenges that attribution methods still face. In this work, we propose: 1) an essential characteristic, Strong Relevance, when selecting attribution features; 2) a new concept, feature map importance (FMI), to refine the contribution of each feature map, which is faithful to the CNN model; and 3) a novel attribution method via FMI, termed A-FMI, to address the gradient saturation problem, which couples the target image with a reference image, and assigns the FMI to the difference-from-reference at the granularity of feature map. Through visual inspections and qualitative evaluations on the ImageNet dataset, we show the compelling advantages of A-FMI on its faithfulness, insensitivity to the choice of reference, class discriminability, and superior explanation performance compared with popular attribution methods across varying CNN architectures.

==> Arxiv2021_ A-FMI/1_introduction.tex <==
\section{Introduction}
% Gradient-based attribution methods are a powerful tool to explain how convolutional neural networks (CNNs) arrive at a particular prediction. To highlight features of an input pertinent to the prediction, two key challenges lie in the 1) the granularity of attribution features and 2) the gradient saturation w.r.t attribution features. However, simply treating image pixels as the attribution features make most methods work as an edge detector, which fails to capture informative regions of interest or relies heavily on the quality of reference pixels. In this work, we propose a novel attribution method, AFMI, to solve the limitations. Instead of using pixels, AFMI harnesses CNN feature maps of an image as its attribution feature, which encourages the local fidelity and global faithfulness of attribution scores. Moreover, AFMI involves the feature map reference, rather than on a granular level of pixels, to help solve the gradient saturation. Hence, it identifies compact regions that have a crucial role in CNN’s prediction. We demonstrate it on interpreting VGG19 in the ImageNet classification task. With thorough visual inspections and qualitative evaluation metrics, extensive experiments show the effectiveness of our approach.

% WX: Attribution methods: definition, a common paradigm involving attribution features * attribution scores = prediction


As the understanding of neural networks is of crucial importance to engender user trust, interpreting network behavior has attracted increasing attention.
To this end, attribution methods~\citep{attribution_method} have demonstrated the remarkable ability in attributing the prediction of a given network, typically CNN, to its input.
% They are typically applied to explain convolutional neural networks (CNNs)~\cite{vgg-19,ResNet} in various applications.
%~\cite{Grad-CAM,DeepLIFT} 
% by highlighting significant regions of an input image to the predicted class.
%Regardless of various designs, we can summarize a common paradigm of existing attribution methods as: 
Regardless of various designs, a common axiom called completeness~\citep{IG} or local-faithfulness~\citep{Grad-CAM} for most existing attribution methods can be summarized as:
$\sum$\emph{attribution feature}$\times$\emph{attribution score}$\approx$\emph{network prediction}.
Simply stated, given an input image, attribution method determines the attribution score (also well-known as relevance~\citep{LRP} or contribution~\citep{LIME}) of each attribution feature (\eg pixel, segment), in order to approximate the CNN's prediction of interest.
% Simply stated, given an input image with a CNN being interpreted, the basic idea is to determine the attribution score (also well-known as relevance~\cite{LRP} or contribution~\cite{LIME}) of each attribution feature (\eg pixel, segment), in order to approximate the CNN prediction of interest. 
By redistributing such attributions to the input image, we can produce a saliency map to highlight the most important regions for predicting the class of interest. 
% By arranging such scores to the input image, we can establish a saliency map to illustrate the influence of the attribution features on the prediction.
% present how attribution features contribute positively or negatively to the prediction.

% Such a score magnitude reflects how the attribute features contribute positively or negatively to the prediction, which can be visually displayed in a saliency map.

% Clearly, to find effective attributions, we need to pay special attention on the selection of attribution feature and the learning of attribution score.


% WX: the granularity of attribution features is of crucial to interpretation.
%     .... two desired properties: relevant, semantic
%     .... popular research lines: pixels vs segments with inherent limitations
%     .... using feature map is of promise


In scrutinizing the axiom, we argue that a key challenge lies in the selection of attribution features, which should satisfy one essential characteristic --- Strong Relevance (a statistic concept in feature selection~\citep{Relevant}). Formally, a strong relevant feature is defined as a feature which has information that is both pertinent to the class prediction and can barely be derived from other features;
in contrast, the redundant feature is highly correlated and can be represented by other features.
Although the redundancy in attribution features does not affect the aprroximation of the prediction, it negatively influences the learning of the attribution scores.
% Though the existence of redundant features does not affect the approximation of the prediction, it negatively influences the learning of the attribution scores.
The key reason is that the entanglement among these features weakens the ability to identify significant features, and small changes of redundant features can swing the value of attribution scores widely.
% Hence, we asset that attribution methods at the granularity of redundant features can easily lead to suboptimal explanations.
% assert; claim; state

% In scrutinizing the paradigm, we argue that a key challenge lies in the selection of attribution features, which should satisfy one essential characteristic --- Relevant. More formally, a relevant feature~\cite{Relevant} is defined as a feature that has information which is both pertinent to the class prediction and hardly derived from other features, in contrast to the redundant feature~\cite{Relevant} that is highly correlated to other features and can be represented by them.
% Assuming some attribution features are redundant, while having no effect on the approximation of the prediction, it negatively influences the learning of attribution scores.
% The key reason is that the entanglement among these features weakens the ability to identify significant features, and small changes of redundant features can swing the value of attribution scores widely.
% Hence, we argue that attribution methods on the granularity of redundant features can easily lead to fragile explanations.

%In a nutshell, the desirable characteristics encourages the attribution features to be maximally compressed about the prediction and filter the redundant signal out.

% 2) Semantic. More specifically, a semantic feature~\cite{LIME,L2X} is defined as one that can be understandable by humans, highlighting the comprehensiveness of explanations.
% For example, in the image classification, single pixels are less appropriate than regions for considering as attribution features; analogously, in the text classification, individual letters in a sentence is of less semantics than words.


% Having realized the vital role of attribution feature selection, we categorize the prior efforts into three groups --- \textbf{pixels}~\cite{gradients,LRP,gradients*input,SmoothGrad,Deconvolution,GuidedBackpropogation,IG,DeepLIFT}, \textbf{regions}~\cite{LIME,PredictionDifferenceAnalysis,XRAI}, and \textbf{feature maps} in the last convolutional layer~\cite{CAM,Grad-CAM,Grad-CAM++}. However, each type of method suffers from some inherent limitations:
% \begin{itemize}
%     \item A research line exploits single pixels as the attribution features, and computes the attribution scores as the gradient~\cite{gradients,gradients*input} or modified gradient~\cite{LRP,DeepLIFT,IG} of the target class \wrt each pixel. Despite great success, the main limitation is that most pixel-wise efforts violate the desired characteristics: First, pixels are redundant since they are strongly related to the surrounding pixels~\cite{PredictionDifferenceAnalysis}. Such redundant attribution features encourage the attribution methods to being akin to the edge detector~\cite{SanityCheck} and make the explanations vulnerable against the pixel-wise perturbations~\cite{fragile}. Second, there is no semantic meaning of single pixels.
%     Furthermore, the significant pixels highlighted in the saliency maps are easily spread out, where the focus shift onto irrelevant edges, objects or even background (\eg Gradient~\cite{gradients} and DeepLIFT~\cite{DeepLIFT} in Figure~\ref{fig:reference}).
    
%     \item Several works focus on the regional segments and compute the attribution of a region by removing it, feeding the new input into the network, and measuring the difference with the original prediction~\cite{LIME,PredictionDifferenceAnalysis}. While region-wise attribution features are semantic meaningful, such perturbation-based methods hardly satisfy the completeness of attributions~\cite{IG} --- that is, adding the attributions of all regions up is hard to match the network prediction.
%     Moreover, the attribution performance heavily depends on the quality of segmentation.
% \end{itemize}

Having realized the vital role of attribution feature selection, we categorize the prior works into three levels of granularity: \textbf{pixels}~\citep{gradients,Deconvolution,GuidedBackpropogation,LRP,gradients*input,SmoothGrad,DeepLIFT,IG,SHAP}, \textbf{regions}~\citep{LIME,PredictionDifferenceAnalysis,MP,real_time_saliency, RISE,EP, XRAI}, and \textbf{feature maps}~\citep{CAM,Grad-CAM,Grad-CAM++}. However, each type of methods suffers from some limitations:
%inherent
\begin{itemize}
    \itemsep0em
    \item One research line exploits single pixels as attribution features and learns the gradients, modified gradients or integrated gradients of the target class as the attribution scores.
    Despite great success, one limitation is that it violates the Strong Relevance characteristic of attribution features, since pixels are strongly related to thier surrounding pixels.
    Such redundancy easily results in suboptimal and fragile attributions, being akin to the edge detector~\citep{SanityCheck} and vulnerable to small perturbations~\citep{fragile}.
    % \item One research line exploits single pixels as attribution features and computes the gradients~\citep{gradients,gradients*input}, modified gradients~\citep{LRP,DeepLIFT} or integrated gradients~\citep{IG} of the target class as the attribution scores.
    % Despite great success, one main limitation is that it violates the Relevance characteristic of attribution features, since pixels are strongly related to the surrounding pixels~\citep{PredictionDifferenceAnalysis}.
    % Such redundancy easily results in suboptimal and fragile attributions, being akin to the edge detector~\citep{SanityCheck} and vulnerable to small perturbations on pixels~\citep{fragile}.
    
    
    
    % Despite its great success, the main limitation is that most pixel-wise efforts violate the desired characteristic of features. Pixels are intrinsically redundant since they are strongly related to the surrounding pixels~\cite{PredictionDifferenceAnalysis}. Such redundant attribution features encourage the attribution methods to be akin to the edge detector~\cite{SanityCheck} and make the explanations vulnerable to small perturbations of the input pixels~\cite{fragile}. Moreover, the significant pixels highlighted in the saliency maps are easily spread out, where the explanation focus shifts into irrelevant edges, objects, or even background (\eg pixel-wise attribution methods in Figure~\ref{fig:introduction}).
    % A research line exploits single pixels as the attribution features, and computes the attribution scores as the gradient~\cite{gradients,gradients*input}, modified gradient~\cite{LRP,DeepLIFT} or integrated gradient~\cite{IG} of the target class \wrt each pixel. Despite great success, the main limitation is that most pixel-wise efforts violate the desired characteristic of features. Pixels are intrinsically redundant since they are strongly related to the surrounding pixels~\cite{PredictionDifferenceAnalysis}. Such redundant attribution features encourage the attribution methods to be akin to the edge detector~\cite{SanityCheck} and make the explanations vulnerable to pixel-wise perturbations~\cite{fragile}. Moreover, the significant pixels highlighted in the saliency maps are easily spread out, where the focus shifts into irrelevant edges, objects, or even background (\eg pixel-wise attribution methods in Figure~\ref{fig:introduction}).
    
    \item Region-level methods measure how sensitive the prediction is to the masked image or perturbations of regional segments.
    % a region in the image and evaluating the difference with the original prediction.
    % \item Several works focus on the regional segments and compute the attribution of a region by masking it, feeding the new input into the network, and measuring the difference with the original prediction~\cite{LIME,PredictionDifferenceAnalysis}. 
    % The main drawback of such perturbation-based solutions is that
    However, they hardly satisfy the completeness principle, \ie adding the attributions of all regions up may not guarantee a match with the prediction. 
    % (like EP and RISE in Figure~\ref{fig:introduction}).
    Moreover, built upon the perturbation or masking mechanism, they are time-consuming and heavily depend on the quality of segmentation.
    
    % the performance of such perturbation-based methods heavily depends on the quality of segmentation, which can be labor-intensive and time-consuming.
    
    \item Decomposing the target prediction to the feature maps in the last convolutional layer via gradient learning has been studied. Compared with pixel-wise attribution methods that easily result in focus shift, feature map-based methods highlight the compact regions of interest (see Figure~\ref{fig:introduction}). We attribute such success to the Strong Relevance characteristic of feature maps, wherein only subtle correlations exist as shown in~\cite{DeepVisualization, FeatureMapRelevant}. However, previous methods inherit gradient saturation problem, which underestimates the contributions and further leading untargeted explanations (see Figure~\ref{fig:framework}).
    
    % The role of feature maps in the last convolutional layer has been studied in the model interpretation.
    % % Another research line exploits the feature maps in the last convolutional layer to interpret the decision of interest.
    % Grad-CAM~\citep{Grad-CAM}, as an effective solution, decomposes the target prediction to the attributions of feature maps via gradient learning.
    % Compared with pixel-wise attribution methods that easily result in focus shift, Grad-CAM highlights the compact regions of interest (see Figure~\ref{fig:introduction}).
    % We attribute such success to the Strong Relevance characteristic of feature maps, wherein only subtle correlations exist as shown in~\cite{DeepVisualization, FeatureMapRelevant}.
    % % among feature maps in the last convolutional layer of CNNs as shown in~\cite{DeepVisualization, FeatureMapRelevant}.
    % However, Grad-CAM inherits the problem of gradient saturation.
    % During the backpropagation, the gradients coming into nonlinear activation functions are likely to approach zero.
    % Such vanishing gradients underestimate the importance of feature maps that have saturated their contribution to the prediction, further leading untargeted explanations (see Figure~\ref{fig:framework}).
    % % Although saturation problem has been studied in the pixel-wise methods like IG~\cite{IG} and DeepLIFT~\cite{DeepLIFT}, it is unexplored in the existing feature map-based methods. 
    
    
    % : as shown in prior efforts~\cite{Grad-CAM, DeepVisualization, FeatureMapRelevant}, there is a redundancy in convolution filters of the lower convolutional layers, while this phenomenon gradually lessens as go deeper, and only a subtle correlation exists in feature maps in the last convolutional layer.
\end{itemize}


% Besides, another research line~\cite{CAM, Grad-CAM, Grad-CAM++} exploits the feature maps in the last convolutional layer to interpret the decision of interest.
% Grad-CAM~\cite{Grad-CAM}, as an effective solution, decomposes the target prediction to the attributions of feature maps via gradient learning.
% Compared with pixel-wise attribution methods that easily result in the focus shift, Grad-CAM highlights the compact regions of interest.
% We attribute such success to the desired Relevant characteristic of feature maps: as shown in prior efforts~\cite{Grad-CAM, DeepVisualization, FeatureMapRelevant}, there is a redundancy in convolution filters of the lower convolutional layers, while this phenomenon gradually lessens as go deeper, and only a subtle correlation exists in feature maps in the last convolutional layer.


\begin{figure}[t]
 \centering
 \includegraphics[width=\textwidth]{chart/introduction.pdf}
 \vspace{-13px}
 \caption{Visual comparison of present attribution methods and the proposed A-FMI at 10\% of important pixels insertion for the prediction of class ``dogsled''. Pixels with significant attributions are remained, while the rest is removed. A black reference is used for DeepLIFT, IG and A-FMI.}
 % Best viewed in color.
 \vspace{-15px}
 \label{fig:introduction}
\end{figure}

% WX: the saturation problem of gradients is under explored on a granular level of feature maps.
%     .... to the best of our knowledge, there is no work.
% However, Grad-CAM inherits the problem of gradient saturation~\cite{IG,DeepLIFT}.
% During the backward pass in the gradient learning, the gradients coming into nonlinear activation functions are likely to be flattened and approach zero.
% Such vanishing gradients underestimate the importance of some feature maps that have saturated their contribution to the prediction, further misleading the explanations.
% Although such a saturation problem has been studied in the pixel-wise methods like IG~\cite{IG} and DeepLIFT~\cite{DeepLIFT}, it is underexplored in the existing feature map-based methods. 

% WX: our work, technical contributions:
%     .... using (CNN feature maps - feature map references) as the attribution features
%     .... using feature map importance (FMI) as the attribution scores. 
% In this work, we pay special attention to the gradient saturation problem on the granularity of feature maps.
% Inspired by pixel-wise solutions~\cite{IG,DeepLIFT}, we hypothesize that introducing the feature map reference could be useful to avoid the vanishing gradients.
% Instead of using feature maps solely, we reconstruct the attribution features by hiring a baseline input (\eg a black image), running a forward pass on the new input, and measuring the differences in the last convolutional layer with the original feature map.
% Built upon the difference-from-reference, we devise \textbf{feature map importance} (FMI) to refine the contribution of each feature map, which is formulated as the modified gradient in Taylor series.
% FMI allows significant feature maps to propagate signal even in situations where their gradients is zero and avoids the discontinuities of gradient.
% Moreover, our FMI satisfies several notable properties: 1) strong representation ability, which embeds the class-specific information and can classify images accurately (evidence in Section~\ref{sec:overall_performance}), 2) local fidelity~\cite{LIME}, which faithfully corresponds how the model arrives the prediction of an instance, and 3) global faithfulness~\cite{LIME}, which finds the feature maps that are globally important (evidence in Section~\ref{sec:overall_performance}).
% We propose a new \textbf{Attribution Method based on FMI} (A-FMI), which is equipped with our difference-from-reference and FMI, to interpret CNN models.
% To validate the effectiveness our A-FMI, we perform thorough visual inspections and qualitative evaluations for VGG19~\cite{vgg-19} on the ImageNet dataset~\cite{ImageNet}.
% The empirical results demonstrate that A-FMI consistently produces better results than other saliency methods.
% In a nutshell, our A-FMI is conceptually advantageous to existing saliency methods in that:
% 1) compared with pixel-wise methods, it uses more relevant attribution features (\ie feature maps), thus outputs compact regions of interest;
% 2) compared with region-level methods, it satisfies the completeness principle and is much efficient \wrt time complexity;
% and 3) compared with feature map-based methods, it solves the gradient saturation problem.

% In this work, we explore the solution to the gradient saturation problem on feature maps.
% Inspired by pixel-wise solutions~\citep{IG,DeepLIFT}, feature map references are introduced to avoid vanishing gradients.
% Instead of using feature maps solely,
In this work, feature map referece is introduced as a solution to the gradient saturation problems.
More specifically, we implement a baseline input (\eg a black image), run a forward pass to get feature map references, and measure the differences with the original feature maps.
To refine the contributions for feature map-based difference-from-references, we devise \textbf{feature map importance} (FMI), which is a set of modified gradients estimated by the Taylor series.
% Built upon the difference-from-reference, we devise \textbf{feature map importance} (FMI) to refine the contribution of each feature map, which is formulated as the modified gradient applying Taylor series.
FMI allows significant feature maps to propagate signals even in situations where their gradients are zero.
Moreover, FMI has notable properties (evidence in Section~\ref{sec:explanation-faithfulness}): 1) strong representation ability, embeding class-specific information which could be directly used to classify, 2) local faithfulness, \ie in the vicinity of the input image, FMI is locally accurate to the CNN.
% Moreover, FMI has several notable properties (evidence in Section~\ref{sec:explanation-faithfulness}): 1) strong representation ability, which embeds the class-specific information, 2) local fidelity, which faithfully corresponds to how the model arrives at the prediction of an instance, and 3) to some extent global faithfulness, which finds the feature maps that are globally important for the target class.

We further propose a new \textbf{Attribution Method via FMI} (A-FMI), which is equipped with difference-from-reference and FMI to interpret the CNN models.
To validate the effectiveness of A-FMI, we perform thorough visual inspections and qualitative evaluations for VGG19 and ResNet50 on the ImageNet dataset.
The empirical results demonstrate that A-FMI consistently produces better results than popular attribution methods and is conceptually advantageous in that:
1) compared with pixel-wise methods, it uses attribution features (\ie feature maps) with Strong Relevance characteristic, thus able to output compact regions of interest; moreover, distinct from other attribution methods who are sensitive to the selection of reference, A-FMI is more robust (evidence in Section~\ref{sec:insensitivity-reference});
2) compared with region-level methods, it satisfies the local faithfulness and is much more efficient;
and 3) compared with feature map-based methods, it inherits the advantage of class discriminability (evidence in Section~\ref{sec:class-discriminability}) and solves the gradient saturation problem, producing more refined and targeted explanations. In summary, this work makes the following contributions:
\begin{itemize}
    \itemsep0em
    \item We emphasize the important role of the selection of attribution features, and compare attribution features into three levels of granularity: pixels, regions, and feature maps \wrt the desirable Strong Relevance characteristic.
    \item To the best of our knowledge, we are the first to introduce the feature map reference and FMI into the attribution methods, to solve the gradient saturation problem.
    \item We conduct extensive experiments, demonstrating the effectiveness and consistency of A-FMI in interpreting VGG-based and ResNet-based architectures on the ImageNet dataset.
\end{itemize}






% %% Background
% Over the course of the past few years, sustained advancements in deep convolutional neural networks (CNNs) have significantly broadened the range of applications of Artificial Intelligence, where real-world computer vision applications include, but are not limited to, image classification~\cite{ResNet,BatchNormalization,AlexNet}, object localization~\cite{OverFeat,R-CNN}, semantic segmentation~\cite{SegNet,DilatedcConvolutions}, and image captioning~\cite{GoogleCaptionGenerator,Visual-SemanticAlignments}. 
% %Though CNNs may provide state-of-the-art results and superior performance, the internal operational mechanisms of CNNs are obscure and the CNN decision making process is uninterpretable by humans. The inability to explain the behaviour and decision making processes of intelligent systems limits their pertinence in risk-sensitive applications. The interpretability of a CNN prediction exposes the features extracted by the network, engenders considerable user trust, facilitates the adoption of the prediction, and allows for straightforward implementation of improvements for the model.
% Though CNNs may provide state-of-the-art results and superior performance, the CNN decision-making process is uninterpretable by humans due to the obscurity of CNN internal operational mechanisms. Therefore, the inability to explain the behaviour and decision-making processes of intelligent systems limits the utilization of CNNs in risk-sensitive applications. An interpretable CNN prediction allows for the display of features extracted by the network, engenders considerable user trust, facilitates the adoption of the prediction, and expedites the straightforward implementation of improvements for the model.   


% % Over the last few years, the encouraging progress of deep convolutional neural networks (CNNs) has opened up impressive Artificial Intelligence capabilities and unprecedented breakthroughs in  a wide variety of real-world computer vision applications, from image classification~\cite{ResNet,BatchNormalization,GoogLeNet,VGG-Net,AlexNet}, to object localization~\cite{OverFeat,R-CNN,FastR-CNN}, semantic segmentation~\cite{SegNet,DilatedcConvolutions}, and image captioning~\cite{GoogleCaptionGenerator,Visual-SemanticAlignments}.
% % However, even, though CNN might provide the current state-of-the-arts result and superior performance, there is little insight into the internal operation. The inability to explain its behavior and decisions limits the effectiveness of today's intelligent system, especially for risk-sensitive applications.
% % Moreover, the ability to interpret a prediction in a CNN reveals the features extracted by the network, engenders considerable user trust, accelerates the adoption, and gives rise to appropriate improvement of model.

% %% Introduction of attribution method
% To rectify the above-mentioned shortcomings, a number of attribution methods have been proposed to attribute the class prediction of a CNN to its original input in order to evaluate the contribution of each pixel. These attribution methods entail the useage of instance-wise saliency maps as a tool to highlight relevant features in an input image. 
% %Before the review of attribution methods, it is important to distinguish between the original image input and features used to explain CNN as well as introduce the desired characteristics of features. 
% Though original input pixels are widely used as attribution features to explain CNN, features can be of many granularities and have varying desired characteristics which must be considered.

% %% The importance of granularity of feature
% % The explanation model must represent data using understandable features regardless of the raw image data.
% % %The explanation model needs to use understandable features in representation data, regardless of the raw image data. 
% % The features that are used to interpret CNN results have differing granularities that range from pixels, regions, to feature maps, therefore the selection of feature granularity can directly and fundamentally influence the transparency and properties of explanation models.
% % % There are different granularities of features for interpreting in CNN such as pixels, regions, and feature maps. The choice of features directly and fundamentally influence transparency and properties of explanation models.
% % The prevailing line of research for CNN interpretability is the exploitation of an understandable linear model due to the fact that model coefficients can directly indicate the feature importance.
% % %One prevalent research line is exploiting an understandable linear model to interpret CNN. Since it is well known that the linear model is truly understood where the coefficients of features in the linear model indicate the feature importance. 
% % However, the reliability of linear explanation model depends on whether it is an appropriate model to analyze the relationships between features and predictions. Namely, the basic assumption of attribution methods reviewed in this paper is that the underlying CNN predictions could be approximate well by a weighted linear sum of features. 

% The explanation model must utilize understandable attribution features to optimally represent the corresponding raw input data. There are differing granularities of attribution features ranging from pixels, regions, to feature maps. The selection of feature granularity is of utmost importance because the granularity directly and fundamentally influences the interpretability and various properties. The prevailing line of research for CNN interpretability entails the exploitation of an easily understandable linear model due to the fact that linear model coefficients can directly indicate the importance of the feature; however, the reliability of using linear models is often questionable. The linear model must be able to analyze the relationship between attribution features and CNN predictions, i.e. the basic assumption of attribution methods reviewed in this paper, underlying CNN predictions could be approximated well by a weighted linear sum of attribution features. This assumption calls into question the validity of the application of linear models in pixel features. 

% %% Characteristics of features
% We now outline the two characteristics of attribution features that are desired - relevant and semantic. 
% 1) A relevant feature is defined as a feature that has information for the prediction that does not exist in any other features. In a linear model, if one feature is highly correlated with many other features, then this feature is redundant in the context of other features as it could be linearly represented by other features. The existence of redundant features in the explanation model will lead to multicollinearity. Severe multicollinearity does not affect the prediction, but it heavily influences the linear model coefficients and, consequently, the interpretability of the explanation model. Therefore, redundant features weaken the ability of explanation models to identify significant features because small changes in input data can swing the value of the coefficients wildly.
% %As a result, irrelevant features reduce the power of the explanation model to identify significant features. 
% 2) A Semantic feature is defined as a feature that can be comprehensible by humans. For example, in the text classification task, possible features are words. Letters in the sentences, as well as incomprehensible embeddings, are not appropriate for considering as features. 

% %% Review & drawbacks of attribution methods: pixel-wise; region-level; feature map based
% Typically, attribution methods can be summarized at three major levels of feature granularity, including pixel-wise, region-level, and feature map based.

% 1) Pixel-wise attribution methods have been extensively studied to identify the effect of pixels on the class prediction~\cite{gradients, LRP, gradients*input, SmoothGrad, Deconvolution, GuidedBackpropogation, IG, DeepLIFT}. Intuitively, when the input data pixels are used as features, the gradients become the coefficients of the linear model. However, a significant disadvantage of the gradient-based attribution methods is saturation problem. 
% %To overcome this problem, a variety of gradient-based attribution approaches use a baseline or reference to evaluate the difference-from-reference and a modified partial derivative to calculate attribution scores, such as DeepLIFT~\cite{DeepLIFT} and Integrated Gradients (IG)~\cite{IG}. However, 
% What is more, pixel-wise attribution methods violate the two characteristics of features. On the one hand, pixels are strongly related to their surrounding pixels. Consequently, a large number of pixels are irrelevant and leading to sensitive explanation results~\cite{fragile}. 
% %It has been shown that even IG pixel-wise attributions are not reliable~\cite{XRAI}. 
% %Also, it is demonstrated in our experiments part that pixel-wise attribution methods tend to learn spurious correlations. 
% On the other hand, there is no semantic meaning for image pixels, and it is hard to figure out the correlation between thousands of significant pixels and predictions~\cite{LIME}. As a result, some pixel-wise gradient-based methods fail to pass the sanity check~\cite{SanityCheck} and cannot be considered completely reliable explanations.

% 2) Attribution methods have also been studied at the granularity of connected and coherent region-level that is semantically meaningful~\cite{LIME, PredictionDifferenceAnalysis, XRAI}.
% %The intuition is simple that make perturbation to patches of image and assess their impact on the prediction. 
% The importance of tightly bounded region of pixels is estimated by constructing a linear function of patches of images. 
% %However, region-level perturbation-based methods could be computationally inefficient as each perturbation requires a forward calculation. 
% However, given the nonlinear operation of CNN, the explanation of region-level attribution methods is only solid for the exact number of features and suitable regions. 

% 3) Apart from the pixel-wise and region-level features, feature maps in the last convolutional layer of CNN are used as features in the explanation model to interpret the decision of interest ~\cite{CAM, Grad-CAM, Grad-CAM++}. The feature maps in the last convolutional layers are expected to have the high-level semantics and relevant information. 
% %The linearity assumption between feature maps and prediction is demonstrated in our experiments. 
% However, the feature map based attribution methods inherit the saturation problem of gradients and not yet solved as far as we know. 

% %% Our method advantages
% Motivated by this challenge, we propose instance-wise Feature Map Importance (FMI) as an embedding of image, and a novel attribution method based on FMI, A-FMI, to produce visual explanations for CNN decisions. The main contribution of this work is twofold:  

% \begin{itemize}
%     \item We propose an instance-wise FMI, which is a reasonable embedding to represent an image. To test the validity of the FMI, we simply use the FMI to classify the images and achieves high accuracy, which demonstrates that FMI implies the property of local fidelity, and also presents to some extent global faithfulness.
%     \item We propose a novel attribution method, A-FMI, that can generate visual explanations from any CNN-based network. In order to address the issue of model saturation, A-FMI compares the feature maps of each image to its feature map reference and replaces simple gradients with FMI. A-FMI is not sensitive to changes in reference and can achieve class discriminability, furthermore, it yields prominent overall performance when compared with other attribution methods.
% \end{itemize}






%Grad-CAM chooses disconnected areas while A-FMI is more refined in the sense that could focus more around the object.
%he results of Grad-CAM tend to become segmented, while the results of A-FMI are more accurate and targeted.

==> Arxiv2021_ A-FMI/2_related_work.tex <==
\section{Related Work}
Pixel-wise attribution methods largely leverage the backpropagation way to redistribute the prediction through the whole CNN model to single pixels.
For example, Gradient \citep{gradients} and Input*Gradient \citep{gradients*input} use gradient of the prediction \wrt each pixel as attribution scores;
DeconvNet~\citep{Deconvolution} and Guided Backpropogation~\citep{GuidedBackpropogation} employ well-designed operations on the gradients of nonlinear activation functions. 
However, the gradient saturation problem is inherent in the backpropagation way, which easily results in the vanishing gradients and underestimating importance of pixels.
To solve this problem, DeepLIFT~\citep{DeepLIFT} employs a baseline (reference) image to calculate the modified partial derivatives of the difference-from-reference as the importance of pixels;
meanwhile, Integrated Gradients (IG)~\citep{IG} aggregates the gradients by gradually varying the input from the baseline to the original image.
Despite great success, the significant pixels highlighted by pixel-wise attribution methods are easily spread out --- that is, the focus of the explanation model shifts into irrelevant edges, objects, or even background (see Figure~\ref{fig:introduction}, pixel-wise attribution methods select top 10\% important pixels including snow and person for label dogsled).


% Pixel-wise attribution methods, known as back-propagating methods, redistribute the prediction score through the whole CNN until the input pixel is reached.
% Saliency map is proposed to use gradients for visualizing the class models~\cite{gradients}.
% DeconvNet~\cite{Deconvolution} and Guided Backpropogation~\cite{GuidedBackpropogation} are closely related to the Gradients~\cite{gradients} except the way handling backpropagation through the nonlinear activation function.
% Nevertheless, when the output of a CNN is nearly saturated, Gradients are highly likely to underestimate the importance of pixels. To tackle this issue, DeepLIFT\cite{DeepLIFT} and LRP\cite{LRP} employ a baseline (\aka reference) image to evaluate the difference-from-reference, and calculate the modified partial derivatives as the importance of pixels;
% meanwhile, Integrated Gradients~\cite{IG} aggregates the gradients by gradually varying input from a baseline to the original input.
% In a word, most pixel-wise attribution methods leverage the network’s modified gradients to quantify the pixel importance~\cite{Towardsbetter}.

Region-level attribution methods combine single pixels into patches or regions, and mainly apply the perturbation mechanism to directly evaluate the marginal effect of each region by masking or replacing it.
For example, LIME~\citep{LIME} approximates the CNN function by a sparse linear model between the patches and prediction, which is learned on perturbations of patches.
Prediction Difference Analysis~\citep{PredictionDifferenceAnalysis} replaces patches with a sample from other images and obtain the contribution of each pixel by averaging the importance of patches containing the pixel.
%Meaningful perturbations~\citep{MP} optimizes a spatial perturbation mask that maximally affects the CNN's output.
% While real-time saliency~\citep{real_time_saliency} uses a neural network to learn the perturbation masks.
RISE~\citep{RISE} randomly occludes an image and weights the changes in the confidence score of CNN.
Extremal Perturbations (EP)~\citep{EP} optimizes a spatial perturbation mask with a fixed area that maximally affects the CNN's output.
XRAI~\citep{XRAI} incorporates the idea of gradients with the region-level features, coalescing smaller regions into larger segments based on the maximum gain of IG per region.
These methods suffer from high computational complexity and heavily rely on the quality of segmentation.

% Region-level attribution methods combines pixels as patches or regions, in order to address the sensitivity and reliability issue in the pixel-wise methods.
% In this research line, perturbation-based methods are widely adopted, which mask a patch and perform a forward pass through the network with the modified image to evaluate the contribution of patches.
% For example,
% LIME~\cite{LIME} approximates the CNN by a sparse linear model between the patches and prediction, learned on perturbations of the original patches.
% Prediction Difference Analysis~\cite{PredictionDifferenceAnalysis} explanations by replacing patches with a sample from other images, so as to obtain a pixel's relevance by averaging the patches containing the pixel.
% However, LIME and Prediction Difference Analysis could be computationally inefficient, since each perturbation requires a forward calculation.
% More recently, XRAI~\cite{XRAI}, a region-level attribution method based on IG, tackles the computational efficiency issues by obtaining maximum gain of integrated gradients per area.

Feature map-based attribution methods use feature maps in the last convolutional layer to produce saliency maps.
Wherein, feature maps capture high-level semantic patterns and spatial information.
CAM~\citep{CAM} replaces the fully-connected layers with a global average pooling layer, and produces a coarse-grained saliency map via a weighted sum of feature maps.
Furthermore, Grad-CAM~\citep{Grad-CAM} uses the average gradients \wrt feature maps as the attribution scores.
Though using gradients is beneficial, Grad-CAM inherits the gradient saturation problem, which is unexplored in the existing feature map-based methods.
%To the best of our knowledge, it is unexplored in the existing feature map-based methods.
In this work, the proposed method, A-FMI, falls within this family and provides a potential solution to the saturation problem.

% Feature map-based attribution methods use feature maps in the last convolutional layer to generate class-speciﬁc saliency map since.
% Wherein, feature maps simultaneously capture high-level semantics constructs and detailed spatial information. CAM~\cite{CAM} replaces the fully-connected layers with global average pooling layer and computes a coarse-grained saliency map via a weighted sum of feature maps.
% % CAM uses CNN weights after the average pooling layer as an indication of the attribution scores of feature maps, by contrast,
% Grad-CAM~\cite{Grad-CAM} uses the gradient information to understand the attribution scores of feature maps. Grad-CAM is a generalization of CAM and does not require specific CNN architecture. However, there is a saturation problem inherent in Grad-CAM. The method proposed in this paper, A-FMI, falls within this family and provides a potential solution of the saturation challenging.


% \begin{itemize}
%     \item A research line exploits single pixels as the attribution features and computes the gradients~\cite{gradients,gradients*input}, modified gradients~\cite{LRP,DeepLIFT} or integrated gradients~\cite{IG} of the target class \wrt pixels as the attribution scores. Despite its great success, the main limitation is that most pixel-wise efforts violate the desired characteristic of features. Pixels are intrinsically redundant since they are strongly related to the surrounding pixels~\cite{PredictionDifferenceAnalysis}. Such redundant attribution features encourage the attribution methods to be akin to the edge detector~\cite{SanityCheck} and make the explanations vulnerable to small perturbations of the input pixels~\cite{fragile}. Moreover, the significant pixels highlighted in the saliency maps are easily spread out, where the explanation focus shifts into irrelevant edges, objects, or even background (\eg pixel-wise attribution methods in Figure~\ref{fig:introduction}).
%     % A research line exploits single pixels as the attribution features, and computes the attribution scores as the gradient~\cite{gradients,gradients*input}, modified gradient~\cite{LRP,DeepLIFT} or integrated gradient~\cite{IG} of the target class \wrt each pixel. Despite great success, the main limitation is that most pixel-wise efforts violate the desired characteristic of features. Pixels are intrinsically redundant since they are strongly related to the surrounding pixels~\cite{PredictionDifferenceAnalysis}. Such redundant attribution features encourage the attribution methods to be akin to the edge detector~\cite{SanityCheck} and make the explanations vulnerable to pixel-wise perturbations~\cite{fragile}. Moreover, the significant pixels highlighted in the saliency maps are easily spread out, where the focus shifts into irrelevant edges, objects, or even background (\eg pixel-wise attribution methods in Figure~\ref{fig:introduction}).
    
%     \item Several works focus on the regional segments and compute the attribution of a region by masking it, feeding the new input into the network, and measuring the difference with the original prediction~\cite{LIME,PredictionDifferenceAnalysis}. The main drawback of such perturbation-based methods is that they hardly satisfy the completeness principle~\cite{IG} (also known as local faithfulness) --- that is, adding the attributions of all regions up may not guarantee a match with the network prediction.
%     Moreover, the attribution performance heavily depends on the quality of segmentation, which can be labor-intensive and time-consuming.
    
%     \item Another research line exploits the feature maps in the last convolutional layer to interpret the decision of interest. Grad-CAM~\cite{Grad-CAM}, as an effective solution, decomposes the target prediction to the attributions of feature maps via gradient learning.
%     Compared with pixel-wise attribution methods that easily result in the focus shift, Grad-CAM highlights the compact regions of interest.
%     We attribute such success to the desired Relevant characteristic of feature maps, wherein only subtle correlations exist between feature maps in the last convolutional layer of CNNs as shown in~\cite{DeepVisualization, FeatureMapRelevant}.
%     However, Grad-CAM inherits the problem of gradient saturation~\cite{IG,DeepLIFT}.
%     During the backward pass in the gradient learning, the gradients coming into nonlinear activation functions are likely to approach zero.
%     Such vanishing gradients underestimate the importance of some feature maps that have saturated their contribution to the prediction, further misleading the explanations.
%     % Although saturation problem has been studied in the pixel-wise methods like IG~\cite{IG} and DeepLIFT~\cite{DeepLIFT}, it is unexplored in the existing feature map-based methods. 
    
    
%     % : as shown in prior efforts~\cite{Grad-CAM, DeepVisualization, FeatureMapRelevant}, there is a redundancy in convolution filters of the lower convolutional layers, while this phenomenon gradually lessens as go deeper, and only a subtle correlation exists in feature maps in the last convolutional layer.
% \end{itemize}

==> Arxiv2021_ A-FMI/3_method.tex <==
% \section{Our method: A-FMI}
% A-FMI solves the model saturation problem discussed in \cite{DeepLIFT,IG} by involving feature map reference and FMI. 

% In a formal setup, $f : \mathcal{R}^P \rightarrow \mathcal{R}^C$ is the original CNN model to be explained, where $C$ is the total number of classes. The local explanation model $S$ designs to interpret a prediction $f(x)$ based on a single instance $x$. Given a specific target class $c$, $S^c$ representing the interpretation for prediction $c$ often uses relevant and semantic feature $A$ that maps to the original inputs through a mapping function $x = h(A)$. Local explainable model tries to ensure $\sum_{i,j} S^c(A_{ij}) \approx f^c(h(A))$ in a neighbour of $A$. In what follows, we elaborate our method, A-FMI, how to explore the saliency map $S_{\text{A-FMI}}^c$ of prediction $c$ w.r.t. feature map $A$. 

% \textbf{Saturation problem matters.}
% As more layers are added to the neural network, some input gradients could approach zero, making the attribution misleading. This vanishing gradient problem occurs even using the ReLU activation function. For a simple example, consider a two-layer ReLU network, $f(\alpha) = ReLU(-ReLU(-\alpha+1)+2)$. Suppose the feature changes from $\alpha = 0$ to $\alpha = 2$, then the function value changes from $f(\alpha=0)=1$ to $f(\alpha=2) = 2$. The contribution of $\alpha$ should be non-zero in this case, but because $f$ flatten at $\alpha=2$, the gradient is $0$ representing that $\alpha$ is not important. To overcome the saturation problem in Grad-CAM, A-FMI introduces feature map reference and FMI. Below we present the intrinsic mathematical reason to use feature map reference and modified weights named FMI.


% \textbf{Intrinsic motivation in math.}
% To simplify the analysis, primarily, we assume the fully connected neural network without taking the structure of feature maps into consideration.
% Let $x^{(l)}$ be the output of layer $l$ for $l=1,2,\cdots, L$, $x^0$ be the input of neural network, and $\sigma$ be the activation function, in a forward pass we have 
% $$y^{(l)} = w^{(l-1)}x^{(l-1)}+b^{(l-1)}$$
% $$x^{(l)}=\sigma(y^{(l)})$$
% where the weight $w^{(l-1)}\in \mathcal{R}^{n_l \times n_{l-1}}$ and the bias $b^{(l-1)} \in \mathcal{R}^{n_l}$. Then for any neuron $j$ in layer $l$, it could be represented as $x_j^{(l)} = \sigma(y_j^{(l)}) = \sigma(\sum_i w_{ji}^{(l-1)}x_i^{(l-1)}+b_j^{(l-1)})$. The partial derivative of neuron $x_j^{(l)}$ with respect to neuron $x_i^{(l-1)}$ is denoted as $\frac{\partial x_j^{(l)}}{\partial x_i^{(l-1)}}=\frac{\partial x_j^{(l)}}{\partial y_j^{(l)}} \cdot \frac{\partial y_j^{(l)}}{\partial x_i^{(l-1)}} = \sigma'(y_j^{(l)})\cdot w_{ji}^{(l-1)}$. The small or zero gradient of activation function $\sigma'(\cdot)$ may cause the gradient vanishing. To conquer this difficulty, using the first order Taylor series, $\sigma'(y_j^{(l)})$ could be estimated with respect to a reference point $y_{j_0}^{(l)}$ as follow
% $$\hat{\sigma'}(y_j^{(l)}) = \frac{\sigma(y_j^{(l)})-\sigma(y_{j_0}^{(l)})}{y_j^{(l)}-y_{j_0}^{(l)}}$$
% Notice that in the case of ReLU, $\hat{\sigma'}(y_j^{(l)}) = \frac{\max\{0,y_j^{(l)}\}-\max\{0,y_{j_0}^{(l)}\}}{y_j^{(l)}-y_{j_0}^{(l)}}\in [0,1]$, and always assigns a value between $(0,1)$ when the signs of $y_j^{(l)}$ and $y_{j_0}^{(l)}$ vary. the estimated gradient equals to zero if and only if both $\sigma(y_j^{(l)})=\sigma(y_{j_0}^{(l)})$, which is reasonable.
% In terms of Tanh, $\frac{\sigma(y_j^{(l)})-0}{y_j^{l}-0} = \frac{1}{y_j^{(l)}} \int_0^{y_j^{(l)}}\sigma'(t)dt $ is the average gradient of the nonlinearity in $[0,y_j^{(l)}]$, which also draws insight into why the estimated gradient of activation function is a potential way to solve the saturation problem. 

% Hence, the difference of neuron $j$ in layer $l$ from the reference could be approximated using all neurons in layer $l-1$ as 
% $$x_j^{(l)}-x_{j_0}^{(l)}=\sum_{i} \frac{\sigma(y_j^{(l)})-\sigma(y_{j_0}^{(l)})}{y_j^{(l)}-y_{j_0}^{(l)}} \cdot w_{ji}^{(l-1)} \cdot (x_i^{(l-1)}-x_{i_0}^{(l-1)})$$
% We define the modified gradient of $x_j^{(l)}$ with respect to $x_i^{(l-1)}$ as $\frac{\partial^{\sigma} x_j^{(l)}}{\partial x_i^{(l-1)}} = \sum_{i} \hat{\sigma'}(y_j^{(l)}) \cdot w_{ji}^{(l-1)}$.
% Similarly, applying chain rule, for any input $x_i^{(0)}$ and prediction score for class $c$, $y^{c}$ (before the softmax) connected through a series of paths $P_{ic}$, the modified gradient is defined as $$\frac{\partial ^{\sigma} y^c}{\partial x_i^{(0)}} = \sum_{p \in P_{ic}} (\prod \hat{\sigma'_{p}} \prod w_{p} )$$

% The difference of $y^c$ from the reference could be approximated using all input in layer $0$ as 
% $$y^c-y_0^c = \sum_i \frac{\partial ^{\sigma} y^c}{\partial x_i^{(0)}} \cdot (x_i^{(0)}-x_{i_0}^{(0)})$$

% \textbf{A-FMI.}
% To obtain the feature map importance (FMI) based saliency map $S_{\text{A-FMI}}^c$ for any class $c$, simply change the single neuron into a feature map. We calculate the modified gradient of the score for class $c$, $y^c$ (before the softmax), with respect to the $k$-th feature map $A^k$, i.e.\ $\frac{\partial^\sigma y^c}{\partial A^k}$. The FMI of a specific feature map $A^k$ regarding class $c$ is an average of all modified gradients in this feature map formulated as
% \begin{equation}
% \begin{split}
%  \text{FMI}_{k}^c & = \frac{1}{N} \sum_{i} \sum_{j} \frac{\partial^\sigma y^c}{\partical A^k_{ij}} \\
%  & = \frac{1}{N} \sum_{i} \sum_{j} \sum_{p \in P} (\prod \hat{\sigma'_{p}} \prod w_{p})
% \end{split}
% \end{equation}
% where $P$ is a set of all paths from any neuron in this feature map $A^k$ to prediction score $y^c$. $\text{FMI}_{k}^c$ is the modified weights of fully connected layers to capture the contribution or importance of feature map $A^k$ in predicting a target class $c$.

% Saliency map $S_{\text{A-FMI}}^c$ defines as a weighted linear combination of the difference between feature maps and their reference feature maps with its corresponding FMI as coefficients as follows
% \begin{equation}
%     S_{\text{A-FMI}}^c = \sum_{k} \text{FMI}_{k}^c \times (A^k - A^{k_0})
% \end{equation}
% where $A^{k_0}$ is a reference feature map of $A^k$. i.e.\ $A^{k_0}$ is the corresponding feature map obtained by performing a forward pass through CNN with a reference image, such as a black or white image. In a word, the saliency map $S_{\text{A-FMI}}^c$ implies the relationship between feature maps and prediction $c$. 

% Noticed that despite the difference in deploying the reference feature maps and modified weights FMI, there is another distinction between Grad-CAM and A-FMI that A-FMI does not apply a ReLU to the linear combination of feature maps. A-FMI cares more about the rank of each pixel instead of highlight only the positive effect for the desired class. No evidence indicates a decrease in localization performance without using ReLU. 




% % Considering a fully-connected neural network where each layer performs a linear transformation $z_j = \sum_{i} w_{ji}x_i + b_{j}$ followed by a nonlinear activation function $x_j=\sigma(z_j)$, the reference in each layer is represented as $x_{j_0}=\sigma(z_{j_0})=\sigma( \sum_{i} w_{ji}x_{i_0} + b_{j})$. 
% % According to the first order Taylor series $\sigma(z_{j_0}) \approx \sigma(z_j) + \sigma'(z_{j})(z_{j_0}-z_j)$, the gradient of activation function could be estimated as $$\hat{\sigma'}(z_j) = \frac{\sigma(z_j)-\sigma(z_{j_0})}{z_j-z_{j_0}}$$.

% % For two neurons $i$ and $j$ in subsequent layers, the difference in one layer output from the reference output could be approximated as $$x_j-x_{j_0}=\hat{\sigma'}(z_j)(z_j-z_{j_0})=\sum_{i} \frac{\sigma(z_j)-\sigma(z_{j_0})}{z_j-z_{j_0}} w_{ji}(x_i-x_{i_0})$$ 
% % where $x_i-x_{i_0}$ is the difference of the input from the reference input, and $\frac{\sigma(z_j)-\sigma(z_{j_0})}{z_j-z_{j_0}} \times w_{ji}$ is the modified gradients $\frac{\partial ^{\sigma} x_j }{\partial x_i}$. 
% % Notice that in the case of ReLU, $\frac{\sigma(z_j)-\sigma(z_{j_0})}{z_j-z_{j_0}} = \frac{\max\{0,z_j\}-\max\{0,z_{j_0}\}}{z_j-z_{j_0}}\in [0,1]$, and assigns a value between $(0,1)$ to solve saturation problem because of the variation of the signs between $z_j$ and $z_{j_0}$.
% % In terms of Tanh, $\frac{\sigma(z_j)-0}{z_j-0}= \frac{1}{z_j} \int_0^{z_j}\sigma'(t)dt $ is the average gradient of the nonlinearity in $[0,z]$, which also draws insight on why the modified gradient could solve the saturation problem. 


\section{Methodology}
% We now present our framework, A-FMI, which introduces the feature map reference into the attribution methods, with the aim of solving the gradient saturation problem.
% In particular, A-FMI hires the difference-from-reference on the granularity of feature map as the attribute features, and creates the feature map importance (FMI) to decompose the CNN prediction of interest.
% Finally, it results in a saliency map to explain how the CNN model arrives at the prediction.

% \subsection{Background \& Problem Formulation}
% We first formulate the task of feature map-based attribution methods and emphasize the inherent gradient saturation problem. We then present a generic solution to the saturation problem in the fully connected neural network and ultimately propose our method A-FMI which takes feature map architecture into consideration.

% We first formulate the task of attributing the prediction on , and emphasize the gradient saturation problem inherent in the gradient-based attribution solutions.

\noindent\textbf{Problem Formulation.}
Let $F$ be the original CNN model that classifies an input image $\Mat{x}$ into one of $C$ classes.
% Let $\Mat{x}$ be an input image, and $F$ be a trained CNN model that classifies $\Mat{x}$ into one of $C$ classes.
The local explanation model designs to interpret $F(\Mat{x})$ consisting of two components: attribution features and attribution scores. 
%We aim to build an attribution model to interpret how the CNN model arrives the prediction $F(\Mat{x})$ at the input $\Mat{x}$.
%It consists of two components: the selection of attribution features and the learning of attribution scores.
We utilize feature maps $\Set{A}$ in the last convolutional layer as the attribution features, obtained by feeding $\Mat{x}$ into the CNN.
%More specifically, by feeding $\Mat{x}$ into the convolutional layers, we obtain its feature maps $\Set{A}$ in the last convolutional layer as our attribution features.
Our goal is to learn the local explanation model (or instance-wise saliency map) $\Mat{S}^{c}(\Set{A})$ for a class of interest $c$ that ensures local faithfulness:  $\sum_{i,j}S^{c}(\Set{A})_{i,j}\approx F^{c}(\Mat{x})$. 
In other words, the sum of entries in the saliency map should approximate the prediction of interest. 
% Given a class of interest $c$ and an input image $\Mat{x}$, our goal is to learn the attribution scores and build the local explanation model (or instance-wise saliency map) $\Mat{S}^{c}(\Set{A})$ that ensures local faithfulness:  $\sum_{i,j}S^{c}(\Set{A})_{i,j}\approx F^{c}(\Mat{x})$. 
% In other words, the local explanation model is required to achieve local faithfulness that the sum of entries in the saliency map should approximate the prediction of interest. 
%To be local faithful, the explanation model must correspond to how CNN predicts in the vicinity of the instance input image.
% Ultimately, we rearrange the attributions to the input data, to obtain saliency map that highlights the significant pixels in visual explanation.


% Given a class of interest $c$, our goal is to establish the saliency map $\Mat{S}^{c}(\Set{A})$, which learns the attribution scores of the attribution features to the CNN output $F^{c}(\Mat{x})$.
% Following the completeness principle~\cite{DeepLIFT,Towardsbetter,SanityCheck}, we formulate the overall objective as $\sum_{i,j}S^{c}(\Set{A})_{i,j}\approx F^{c}(\Mat{x})$ --- more specifically, using the sum of entires in the saliency map to approximate the prediction of interest.
% Ultimately, we arrange the saliency map to the input data, to highlight the significant pixels in visual inspections.



% Let $\Mat{x}\in\Space{R}^{D}$ denote an input associated with a $D$-dimensional features, and $F: \Space{R}^{D}\rightarrow\Space{R}^{C}$ be a trained classifier model that maps $\Mat{x}$ into one of $C$ classes.
% An attribution method $S$ is to interpret how the classifier model arrives the prediction $F(\Mat{x})$ at the input $\Mat{x}$.
% It typically consists of three components: the selection of attribution features, the learning of attribution scores, and the construction of saliency map.
% More specifically, by applying a mapping function $H$ on $\Mat{x}$, an attribution method constructs the attribution features $\Mat{A}=H(\Mat{x})\in\Space{R}^{D'}$, which can be set as pixels~\cite{DeepLIFT,IG}, regional segments~\cite{LIME,XRAI}, feature maps in the last convolutional layer~\cite{Grad-CAM}, or outputs of any internal layers.
% Given a class $c$ of interest, the goal is to determine the contribution $S^{c}(\Mat{A})=[S^{c}(A_{1}),\cdots,S^{c}(A_{D'})]\in\Space{R}^{D'}$ of each attribution feature $A_{i}$ to the model prediction $F^{c}(\Mat{x})$.
% More formally, the objective is $\sum_{i}S^{c}(A_{i})\approx F^{c}(\Mat{x})$.
% Ultimately, the saliency map $M:\Space{R}^{D'}\rightarrow\Space{R}^{D}$ is constructed by arranging the attribution scores $S^{c}(\Mat{A})$ to the input data.

\noindent\textbf{Gradient Saturation Problem.}\label{sec:saturation-problem}
Exploiting the gradients of attribution features \wrt the target class as attribution scores is a prevalent technique in the existing attribution methods.
However, the problem of gradient saturation is inherent in the gradient learning process, which easily leads to suboptimal attribution scores.
% Exploiting the gradients of each attribution feature \wrt the target class is a prevalent technique in the existing attribution methods.
% However, the problem of gradient saturation is inherent in the gradient learning process, easily leading to suboptimal attribution scores.
The key reason is that, during the backward pass, vanishing gradients may occur due to nonlinear activation functions (\eg sigmoid, tanh, and even ReLU).
Taking a two-layer ReLU network $F(\alpha)=\text{ReLU}(-\text{ReLU}(-\alpha+1)+2)$ as an example, the gradient of $F(\alpha)$ at $\alpha=2$ is $0$, intuitively indicating its trivial contribution.
However, when changing $\alpha$ from $0$ to $2$, the network output changes from $F(\alpha=0)=1$ to $F(\alpha=2)=2$, which suggests that $\alpha$ is significant for prediction.
% This inspires researchers~\cite{IG,DeepLIFT} to introduce the reference (\eg $A=0$ in the toy example) to measure the attribution, instead of gradient merely.
Clearly, such vanishing gradients easily mislead the learning of attribution scores.
Hence, It is of crucial importance to solve the gradient saturation problem.



% \subsection{Our Solution}
% We conclude this section with a discussion on the relation with Grad-CAM.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{chart/framework.pdf}
    \vspace{-13px}
    \caption{Overview (left) and Visual Comparisons (right) between Grad-CAM and A-FMI.} 
    \vspace{-15px}
    \label{fig:framework}
\end{figure}

\noindent\textbf{Mathematical Motivation.}
For clarification of presentation, let us first consider a network that only consists of $L$ fully connected layers as the classifier being interpreted, while first leaving the feature maps untouched.
Let $\Mat{x}^{(0)}\in\Space{R}^{d_{0}}$ denote the input vector associated with $d_{0}$-dimensional features, and $\Mat{y}^{(L)}\in\Space{R}^{C}$ be the prediction over $C$ classes in the last layer (before softmax).
In a forward pass, the output of each layer $\Mat{x}^{(l)}$ is modeled as:
% $\Mat{x}^{(l)}=\sigma{(\Mat{y}^{(l)})},\quad\Mat{y}^{(l)}=\Mat{W}^{(l)}\Mat{x}^{(l-1)} + \Mat{b}^{(l)},$
\begin{equation}
    \Mat{x}^{(l)}=\sigma{(\Mat{y}^{(l)})},\quad\Mat{y}^{(l)}=\Mat{W}^{(l)}\Mat{x}^{(l-1)} + \Mat{b}^{(l)}
\end{equation}
where $\Mat{W}^{(l)}\in\Space{R}^{d_{l}\times d_{l-1}}$ and $\Mat{b}^{(l)}\in\Space{R}^{d_{l}}$ are the weight matrix and bias terms in the $l$-th layer; $\sigma(\cdot)$ is a nonlinear activation function; and $d_{l}$ is the dimension of the $l$-th layer.
Obviously, the $j$-th neuron in the $l$-th layer is represented using all neurons in the previous layer as: $x_j^{(l)} = \sigma(y_j^{(l)}) = \sigma(\sum_i W_{ji}^{(l)}x_i^{(l-1)}+b_j^{(l)})$.
% Obviously, the $j$-th neuron in the $l$-th layer is derived from the weight paths connecting the neuron and all neurons in the previous layer --- that is, $x_j^{(l)} = \sigma(y_j^{(l)}) = \sigma(\sum_i W_{ji}^{(l)}x_i^{(l-1)}+b_j^{(l)})$.
Hence, to measure the contribution of the $i$-th neuron in ($l$-1)-th layer (\ie $x^{(l-1)}_{i}$) to the $j$-th neuron in the subsequent layer (\ie $x^{(l)}_{j}$), an intuitive solution is to leverage the partial derivative as:
$\frac{\partial x_j^{(l)}}{\partial x_i^{(l-1)}}=\frac{\partial x_j^{(l)}}{\partial y_j^{(l)}} \cdot \frac{\partial y_j^{(l)}}{\partial x_i^{(l-1)}} = \sigma'(y_j^{(l)})\cdot W_{ji}^{(l)}$.
However, when $\sigma(y_j^{(l)})$ is flatten, $\sigma'(y_j^{(l)})$ approaches zero which may underestimate the contribution. To avoid unreasonable gradient vanishing, we employ the first order Taylor series to better estimate $\sigma'(y_j^{(l)})$ using a reference point $\bar{y}_{j}^{(l)}$, as: 
% To better estimate the value of $\sigma'(y_j^{(l)})$ and avoid unreasonable gradient vanishing, we employ the first order Taylor series to create an estimator $\hat{\sigma'}(y_j^{(l)})$.
% In particular, beyond the point $y_{j}^{(l)}$, we introduce a reference point $\bar{y}_{j}^{(l)}$, run a forward pass with the reference, and measure the ratio between the differences in output and input, as:
\begin{equation}
    \hat{\sigma'}(y_j^{(l)}) = \frac{\sigma(y_j^{(l)})-\sigma(\bar{y}_{j}^{(l)})}{y_j^{(l)}-\bar{y}_{j}^{(l)}}
\end{equation}
% where $\sigma(y_j^{(l)})-\sigma(\bar{y}_{j}^{(l)})$ and $y_j^{(l)}-\bar{y}_{j}^{(l)}$ are the difference-from-reference in input and output of the activation function, respectively.
Here we use two cases to illuminate how the estimation process is of promise to solving the saturation problem:
1) When the activation function is ReLU,
$\hat{\sigma'}(y_j^{(l)}) = \frac{\max\{0,y_j^{(l)}\}-\max\{0,\bar{y}_{j}^{(l)}\}}{y_j^{(l)}-\bar{y}_{j}^{(l)}}$.
It always assigns a value in a range of $(0,1)$ when the signs of $y_j^{(l)}$ and $\bar{y}_{j}^{(l)}$ are different; and it is zero if and only if $\sigma(y_j^{(l)})=\sigma(\bar{y}_{j}^{(l)})$.
2) When the activation function is tanh, we set the reference as 0 for simplicity and have
$\hat{\sigma'}(y_j^{(l)}) = \frac{1}{y_j^{(l)}} \int_0^{y_j^{(l)}}\sigma'(t)dt$,
% $\hat{\sigma'}(y_j^{(l)}) = (1/ y_j^{(l)})\cdot \int_0^{y_j^{(l)}}\sigma'(t)dt $.
which is the average gradient of the nonlinearity in $[0,y_j^{(l)}]$.
These estimators show the ability in identifying the significant features by assigning a non-zero value and filtering the irrelevant ones out by outputting a zero value.

Having established the estimator $\hat{\sigma'}(y_j^{(l)})$, we are able to approximate the difference of neuron $x_j^{(l)}$ from its own reference $\bar{x}_{j}^{(l)}$ in the $l$-th layer using all neurons in the ($l$-1)-th layer as follows:
\begin{gather}
    x_j^{(l)}-\bar{x}_{j}^{(l)}=\sum_{i} \hat{\sigma'}(y_j^{(l)}) \cdot w_{ji}^{(l)} \cdot (x_i^{(l-1)}-\bar{x}_{i}^{(l-1)})
\end{gather}
Consequently, we can define the modified gradient of the $l$-layer's output $x_j^{(l)}$ \wrt $x_i^{(l-1)}$ as $\frac{\partial^{\sigma} x_j^{(l)}}{\partial x_i^{(l-1)}} = \sum_{i} \hat{\sigma'}(y_j^{(l)}) \cdot w_{ji}^{(l)}$.
We further apply the chain rule of gradient to estimate the attribution of the original input $x_i^{(0)}$ to the final prediction $y^{(L)}_{c}$ of the last layer (before softmax) as:
\begin{gather}\label{equ:generic-attribution-score}
    \frac{\partial ^{\sigma} y^{(L)}_{c}}{\partial x_i^{(0)}} = \sum_{p \in \Set{P}} (\prod \hat{\sigma'_{p}} \prod W_{p})
\end{gather}
where $\Set{P}$ is the set of paths that connect the $i$-th neuron in the input (\ie $x_i^{(0)}$) with the $c$-th neuron in the last layer (\eg $y^{(L)}_{c}$).
Iteratively, in the last layer, the difference between $y^{(L)}_{c}$ and its reference $\bar{y}^{(L)}_{c}$ can be successfully fetched by a weighted sum of all inputs:
% Iteratively, in the last layer, the difference of $y^{(L)}_{c}$ from the prediction of reference $\bar{y}^{(L)}_{c}$ can be successfully fetched by a weighted sum of input:
\begin{gather}\label{equ:generic-attribution-objective}
    y^{(L)}_{c} - \bar{y}^{(L)}_{c}=\sum_i \frac{\partial ^{\sigma} y^{(L)}_{c}}{\partial x_i^{(0)}} \cdot (x_i^{(0)}-\bar{x}_{i}^{(0)})
\end{gather}
An image that has no specific information for any class, \ie has a near-zero prediction score, can be a proper reference. This encourages the sum of attributions to approximate the prediction of interest. 
Moreover, unlike previous studies that mostly treat instance-wise baselines as hyper-parameters and need to carefully select them (\eg adversarial examples or blurred images) to improve the explanation quality, we simply fix an identical reference for all images, to which our attribution scores are insensitive.
% Moreover, distinct from previous studies that a good instance-wise baseline (like adversarial example or blurred image) should be carefully selected to improve the explanation, we think a reference is a factor that does not contribute to the model prediction and hence should not significantly affect the explanation as well as should be identical for all images to be fair.
% Selecting a proper reference input makes its prediction $y^{(L)}_{c_{0}}$ approach zero, thus can encourage the attribution sum to approximate the prediction of interest $y^{(L)}_{c}$. 


\noindent\textbf{Attribution Method via FMI (A-FMI).}
Having obtained the potential solution to the gradient saturation problem, we subsume our feature map-based attribution method under this solution, as Figure~\ref{fig:framework} shows.
Distinct from Grad-CAM that only takes the target image as input, we additionally couple it with a reference image (\eg a black image) and feed them into the CNN model.
The CNN model yields the feature maps $\Set{A}=\{\Mat{A}^{k}\}$ with the feature map references $\bar{\Set{A}}=\{\bar{\Mat{A}}^{k}\}$ in the last convolutional layer, and the outputs $\{\Mat{x}^{(L)}\}$ and output references $\{\bar{\Mat{x}}^{(L)}\}$ (before softmax) in the last fully-connected layers.
Thereafter, to obtain the $\text{FMI}_{k}^{c}$ of the $k$-th feature map $\Mat{A}^{k}\in\Set{A}$ to the target prediction $y_{c}^{(L)}$, we simply change the single neuron $x^{(0)}_{i}$ in Equation~\eqref{equ:generic-attribution-score} with the entry of $\Mat{A}^{k}_{ij}$ and average all modified gradients in the feature map $\Mat{A}^{k}$, which is formulated as follows:
% First, to obtain the feature map importance (FMI) of the $k$-th feature map $\Mat{A}^{k}\in\Set{A}$ to the target prediction $y_{c}$, we simply change the single neuron $x^{(0)}_{i}$ in Equation~\eqref{equ:generic-attribution-score} with the entry of $\Mat{A}^{k}$ and average these modified gradients, which is formulated as follows:
\begin{gather}\label{equ:fmi}
    \text{FMI}_{k}^{c} = \frac{1}{N} \sum_{i} \sum_{j} \frac{\partial^{\sigma} y_c^{(L)}}{\partial A^k_{ij}} = \frac{1}{N} \sum_{i} \sum_{j} \sum_{p \in P} (\prod \hat{\sigma'_{p}} \prod W_{p}),
\end{gather}
where $A_{ij}^{k}$ is the entry of $\Mat{A}^{k}$ located in the $i$-th row and $j$-th column; $N$ is the total number of entries in the feature map $\Mat{A}^{k}$; and $\Set{P}$ is the set of paths starting from any neuron in this feature map to the prediction score $y_{c}^{(L)}$.
In essence, $\text{FMI}_{k}^c$ is the modified weight of the fully connected layers in the CNN model, which directly captures the contribution of feature map $\Mat{A}^{k}$ in predicting target class $c$. 

% With the FMI scores of feature maps $\{\text{FMI}_{k}^c|\Mat{A}^{k}\in\Set{A}\}$, the overall
The saliency map $S_{\text{A-FMI}}^c$ is modeled as a weighted linear combination of the difference between the feature maps $\{\Mat{A}^{k}\}$ and feature map references $\{\Mat{\bar{A}}^{k}\}$ with the corresponding $\text{FMI}_{k}^c$ scores as the coefficients.
More formally, the weighted combination can be represented as follows:
\begin{equation}
    \Mat{S}_{\text{A-FMI}}^c = \sum_{k} \text{FMI}_{k}^c \cdot (\Mat{A}^k - \Mat{\bar{A}}^{k})
\end{equation}
Note that feature map importance $\text{FMI}_{k}^c$ differs from the importance weights in Grad-CAM.  
% Note that $\Mat{S}_{\text{A-FMI}}^c$ indicates the relationship between feature maps and the prediction.
% which essentially fits Equation~\ref{equ:generic-attribution-objective} and reveals the relationship between feature maps and the prediction.


% Noticed that despite the difference in deploying the reference feature maps and modified weights FMI, there is another distinction between Grad-CAM and A-FMI that A-FMI does not apply a ReLU to the linear combination of feature maps. A-FMI cares more about the rank of each pixel instead of highlight only the positive effect for the desired class. No evidence indicates a decrease in localization performance without using ReLU. 





==> Arxiv2021_ A-FMI/4_experiments.tex <==
% \section{Experiments}
% In this section, we conduct extensive experiments to answer the following four research questions:
% \begin{itemize}
%     \item \textbf{RQ1}: Are the explanations of A-FMI faithful to the CNN model?
%     \item \textbf{RQ2}: How do different reference images affect the explanations of A-FMI? 
%     \item \textbf{RQ3}: Can A-FMI distinguish between different classes of interest?
%     % \item \textbf{RQ3}: Can A-FMI distinguish between classes?
%     \item \textbf{RQ4}: How does A-FMI perform compared with popular attribution methods?
%     %Compared with present attribution methods, how does A-FMI perform?
% \end{itemize}

% To answer RQ1, we qualitatively evaluate the faithfulness of A-FMI to the VGG19~\cite{vgg-19} model on the ImageNet~\cite{ImageNet} validation images, as well as a simple CNN model on the MNIST~\cite{MNIST} validation set.
% To answer the remaining questions, we evaluate and compare A-FMI to other popular attribution methods \wrt visual inspections and qualitative metrics, validating the effectiveness in terms of insensitivity to the reference, class discriminability, and explanation quality.
% To ensure the reproducibility, we have uploaded the codes of A-FMI and other attribution methods in the supplementary material.
% Please see the supplementary material for more details.

\section{Experiments}
In this section, we conduct extensive experiments to answer the following four research questions:
\begin{itemize}
    \itemsep0em
    \item \textbf{RQ1}: Are the explanations of A-FMI faithful to the CNN model?
    \item \textbf{RQ2}: How do different reference images affect the explanations of A-FMI? 
    \item \textbf{RQ3}: Can A-FMI distinguish between different classes of interest?
    % \item \textbf{RQ3}: Can A-FMI distinguish between classes?
    \item \textbf{RQ4}: How does A-FMI perform compared with other popular attribution methods?
    %Compared with present attribution methods, how does A-FMI perform?
\end{itemize}

To answer RQ1, we qualitatively evaluate the faithfulness of A-FMI to the VGG19~\citep{vgg-19} model on the ImageNet~\citep{ImageNet} validation set, as well as a simple CNN model~\citep{pytorch_cnn} on the MNIST~\citep{MNIST} validation set, where only correctly predicted images are considered (\cf Section~\ref{sec:explanation-faithfulness}).
To answer the remaining questions, we compare A-FMI to popular attribution methods:
pixel-wise (Gradient, DeepLIFT, IG, LRP),
region-level (XRAI, EP, RISE), and feature map-based (Grad-CAM).
Without specification, we use a black image as the reference in DeepLIFT, IG, and A-FMI.
% and show sample explanations of the VGG19. 
Visual inspections on VGG19 and qualitative metrics on both VGG19 and ResNet50~\citep{ResNet} are used to validate the effectiveness of A-FMI in terms of reference reliability (\cf Section~\ref{sec:insensitivity-reference}), class discriminability (\cf Section~\ref{sec:class-discriminability}), and explanation quality (\cf Section~\ref{sec:overall-performance}). 
To ensure the reproducibility of our work, we have uploaded the code of A-FMI, all baselines, and their comparisons in the supplementary material.
% See visualization of A-FMI on ResNet~\citep{ResNet} in Appendix B.


% To answer RQ1, we qualitatively evaluate the faithfulness of A-FMI to the VGG19~\cite{vgg-19} model on the ImageNet~\cite{ImageNet} validation set, as well as a simple CNN model~\cite{pytorch_cnn} on the MNIST~\cite{MNIST} validation set (\cf Section~\ref{sec:explanation-faithfulness}).
% As for the remaining questions, we compare A-FMI to popular attribution methods on three granular levels of attribution features: pixel-wise (Gradient~\cite{gradients}, DeepLIFT~\cite{DeepLIFT} with various references, IG~\cite{IG} with various references, LRP~\cite{LRP}), region-level (XRAI~\cite{XRAI} with the white-black reference), and feature map-based (Grad-CAM~\cite{Grad-CAM}) on the ImageNet.
% Visual inspections and qualitative metrics are used to validate the effectiveness of A-FMI in terms of reference reliability (\cf Section~\ref{sec:insensitivity-reference}), class discriminability (\cf Section~\ref{sec:class-discriminability}), and explanation quality (\cf Section~\ref{sec:overall-performance}). 
% Without specification, the black reference are used in DeepLIFT, IG and A-FMI; and VGG19 are interpreted in visualization.
% To ensure the reproducibility of our work, we have uploaded the code of A-FMI, all baselines, and their comparisons in the supplementary material.
% See the supplementary material for more details.



% To answer RQ1, we use two publicly available datasets: MNIST~\cite{MNIST} and ILSVRC2012~\cite{ImageNet}. A pre-trained off-the-shelf VCG-19 model~\cite{vgg-19} and a self-trained convolutional neural network (architecture shown in Appendix) are used for the ImageNet and MNIST datasets, respectively. 

% To answer Q2-4, we select the sample images from ILSVRC2012 and evaluate pre-trained VGG-19. Comparative analyses are conducted for the results of A-FMI and six other state-of-the-art explanation methods. 
% The six other state-of-the-art attribution methods include pixel-wise attribution methods: Gradients, DeepLIFT with varying references, Integrated Gradients (IG) with varying references, Layer-wise Relevance Propagation (LRP); region-level attribution method: XRAI with the white and black reference; and feature map based method: Grad-CAM.

% \subsection{Faithfulness of Explanation (RQ1)}\label{sec:FMI_classification}
% % Faithfulness of explanation model is its ability to accurately explain the function learned by the CNN. To the best of our knowledge, there is no present attribution method proving its global faithfulness. Since a linear explanation model is hard to be the entire description of nonlinear function of CNN, especially for those attribution methods who select pixels or regions as features. Only the local fidelity is expected and checked among attribution methods, \ie in the vicinity of the instance input image, the explanation model must correspond to how the CNN predicts. We evaluate how faithful A-FMI is to CNN from both local and global perspectives by using FMI to classify the images.

% The faithfulness of an explanation model is determined by the ability of the model to accurately explain the function learned by CNN. To the best of our knowledge, none of the current attribution methods have been verified to have the property of global faithfulness because the linear explanation models are hard to provide an entire description of nonlinear CNN functions. Global faithfulness is especially difficult to attain by the attribution methods at granularities of pixels or regions, and only local fidelity is expected of these attribution methods. To be local faithful, the explanation model must correspond to how CNN predicts in the vicinity of the instance input image. In this experiment, we evaluate the faithfulness of A-FMI from both a local and global perspective by classifying images using FMI.   

% % The basic idea behind this experiment is that if the feature map is the appropriate feature to construct an explanation model, then the set of attribution scores (FMI) for a target class should be a meaningful representation for the instance image. In the same class, a common pattern is expected to occur which means some feature maps should be globally important to figure out the specific class. Motivated by this, for a specific image in class $c$, we use the attribution scores of feature maps $\text{FMI}^c = \{\text{FMI}_1^c, \cdots, \text{FMI}_{K}^c\}$ as the embedding of the image. The class-wise mean $\text{FMI}^c$ in the training set is calculated and cosine similarity is used as a metric to classify the images in the validation set. Here, we only consider the images that CNN is able to make the correct prediction. Impressively, when the image is correctly classified by CNN in target $c$ class, its $\text{FMI}^c$ has an extremely high similarity with class-wise mean $\text{FMI}^c$. We achieve outstanding \textbf{86.9\%} and \textbf{88.4\%} accuracy in MNIST and ImageNet dataset among 10 and 1000 distinct classes respectively. 
% % The results illustrate that for each image, its $\text{FMI}^c$ is a qualified representation and also contains class information where similar class images are closer to one another. Speaking more broadly, this essential experiment demonstrates that feature maps are relevant features and our instance-wise explanation is locally faithful. Moreover, the summarized mean of $\text{FMI}^c$ reveals to some extent a global faithful explanation.

% The basic idea of this experiment is that if the feature map is the appropriate feature to construct an explanation model, then the set of attribution scores (FMI) for a target class should be able to meaningfully represent an instance image. Therefore, we hypothesize that a similar pattern should be present for attribution scores of the same class, which means that some feature maps should be globally important to figure out the specific class. Motivated by our hypothesis, we use the attribution scores of feature maps as the embedding of a specific image in class $c$, wherein $\text{FMI}^c = \{\text{FMI}_1^c, \cdots, \text{FMI}_{K}^c\}$. The class-wise mean $\text{FMI}^c$ in the training set is calculated and cosine similarity is used as a metric to classify the images in the validation set, where we only consider images that are correctly predicted by CNN. Impressively, when the image is correctly classified by CNN in target $c$ class, its $\text{FMI}^c$ has an extremely high similarity with class-wise mean $\text{FMI}^c$. The results of the experiment show that we have achieved an outstanding  \textbf{86.9\%} and \textbf{88.4\%} accuracy with 10 distinct classes in MNIST and 1000 distinct classes in ImageNet datasets, respectively.
% In summary, instance-wise $\text{FMI}^c$ is qualified to be a representation of an image and it also contains class information where similar class images are close to one another.  Speaking more broadly, this essential experiment demonstrates that feature maps are relevant features and our instance-wise explanation is locally faithful and the summarized mean of $\text{FMI}^c$ has some extent of global faithfulness. 

\subsection{Faithfulness of Explanation (RQ1)}\label{sec:explanation-faithfulness} 
The faithfulness of an explanation model is its ability to accurately estimate the function learned by the CNN model.
Typically, it can be described on two levels: 1) local faithfulness, justifying whether the explanations corresponds to the CNN predictions in the vicinity of an image instance, and 2) global faithfulness, validating whether the globally important features for a target class are identified.
However, as the evaluation of global faithfulness is seldom performed in existing attribution methods, no measuring framework is available.
Hence, we propose a measuring framework which uses FMI to classify the images to evaluate the faithfulness of A-FMI from both local and global perspectives.


To this end, for a specific image in class $c$, we use the attribution scores of its feature maps $\text{FMI}^c = \{\text{FMI}_1^c, \cdots, \text{FMI}_{K}^c\}$ as the refined representation of the image.
We then average the class-specific attribution scores over all training images as $\overline{\text{FMI}}^c$, which can be viewed as the representation of the prototype in class $c$.
Thereafter, we classify each image in the validation set based on its cosine similarity with the prototype representations $\{\overline{\text{FMI}}^1,\cdots,\overline{\text{FMI}}^C\}$.
If the FMI-based class is identical to the target class $c$, the explanation of an image is faithful to the CNN model.
Impressively, we achieve an average explanation accuracy of \textbf{86.9\%} and \textbf{88.4\%} in MNIST with 10 classes and ImageNet datasets with 1000 classes, respectively.

We present a faithfulness analysis of A-FMI based on the classification accuracy.
First, the instance-wise $\text{FMI}^c$ is well qualified to be a representation of an image, which encodes the information pertinent to the class $c$ from a single image and hence reflects the local faithfulness.
Then, the cosine similarity-based accuracy indicates that images with the same classes tend to form clusters, and the prototype representation $\overline{\text{FMI}}^c$ captures the class-wise patterns.
This further suggests that A-FMI to some extent achieves the global faithfulness.

% \subsection{Reference reliability (RQ2)}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{chart/reference.pdf}
%     \vspace{-15px}
%     \caption{\textbf{Reference reliability.} A-FMI is reliable and robust to the different choices of reference. In contrast, both DeepLIFT and IG determine the attribution strongly relative to a chosen reference. B, W, and R stand for black reference, white reference, and random reference respectively.}
%     \vspace{-15px}
%     \label{fig:reference}
% \end{figure}

% It is well known that constructing an interpretation for CNN is not enough. The explanation itself must be robust to factors that do not contribute to the model prediction in order to establish human trust. When it comes to the state-of-art methods DeepLIFT and IG, which both use references to solve the saturation problems, we evaluate their robustness and reliability of selecting various references. 

% It could be easily observed in Figure~\ref{fig:reference} that the important pixels selected by Deeplift and IG are very spread out, however, in reality, pixels of the object of interest are connected in a continuous mass.
% %the pixels adjacent to the important pixels should most likely also be important. 
% Therefore, interpreting important pixels in a spread-out nature to explain an object of interest with a concentrated and continuous mass will inevitably yield an explanation that is both unclear and unfocused. Furthermore, DeepLIFT and IG will focus on the background and irrelevant objects. Whereas A-FMI explanations are patterned in a manner that is conducive to the clear and focused illustration of the object of interest. For example, a large portion of the important pixels of DeepLIFT, and for a lesser part IG, are located on the branch and the grass (2nd row); whereas, A-FMI will only begin to label irrelevant pixels as important pixels once the entire object of interest has been identified. 

% The selection of reference, such as black (B), white (W), random (R), significantly affects the outcome of Deeplift and IG, whereas A-FMI is not sensitive to changes in reference. 
% White reference tends to favor the attribution of darker pixels in both DeepLIFT and IG; for example, their saliency maps have entirely ignored the object of interest when processing the image of the white dog (1st row). Whereas, the black reference tends to favor the attribution of lighter pixels in both DeepLIFT and IG; for example, they focus more heavily on the white background surrounding the green apples rather than the 
% class itself (3rd row). When utilizing a random reference, the results of DeepLIFT are unsatisfactory (4th column); while, the performance of IG is entirely nonsensical (7th column).

% In conclusion, A-FMI is not susceptible to the choice of the reference image, on the contrary, the change of reference could dramatically diverge the attribution of DeepLIFT and IG. In other words, the selection of reference is just a prior by the A-FMI rather than a hyperparameter in DeepLIFT and IG. It is an advantage property for A-FMI since the reference choice should be guaranteeing reliability without hinging on instance-by-instance solutions~\cite{input_invariance}. More examples of reference unreliability of DeepLIFT and IG are also depicted in the Appendix. 

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{chart/reference.pdf}
    \vspace{-10px}
    \caption{\textbf{Reference reliability.} A-FMI is reliable for the different choices of reference, while both DeepLIFT and IG determine the attribution strongly relative to a chosen reference. B, W, and R stand for black, white, and random reference respectively. See more samples in Appendix C.} 
    \vspace{-15px}
    \label{fig:reference}
\end{figure}

\subsection{Reference Reliability (RQ2)}\label{sec:insensitivity-reference}
To engender user trust, a reliable and trustworthy explanation model should be robust to factors that do not contribute to the model prediction.
Hence, we explore how the reference, a factor additionally introduced to solve the saturation problem, affects DeepLIFT, IG, and A-FMI.
Accordingly, we consider the variants of A-FMI, DeepLIFT, and IG that use different references --- a black image, a white image, and an image filled with random pixels to produce saliency maps in Figure~\ref{fig:reference}.
% Towards this end, we consider the variants of A-FMI that uses different references --- more specifically, a black image, a white image, and a image filled with random pixels --- termed as A-FMI(B), A-FMI(W), and A-FMI(R), respectively.
% Similar notations are used for DeepLIFT and IG.
% We illustrate the saliency maps of A-FMI with DeepLIFT and IG in Figure~\ref{fig:reference} with three images, and have several observations.
% A reliable and trustworthy explanation model should be robust to factors that do not contribute to the model prediction, in order to engender user trust.
% Hence, we explore how the reference, a factor additionally introduced to solve the saturation problem, affects DeepLIFT, IG, and A-FMI, in terms of saliency map, robustness, and reliability of explanations.


% Regardless of references, DeepLIFT and IG create grainy saliency maps and focus more attributions on the background or irrelevant objects (\eg the branch and grass highlighted in the 2nd row) than within the objects of interest (\eg the bird).
% Whereas, A-FMI produces smooth and compact regions, which cover the objects of interest well.
% This visually demonstrates that the DeepLIFT and IG suffer from the spread-out nature since the pixels are naturally redundant and violate the Relevant characteristic of attribution feature.

% Regardless of references, DeepLIFT and IG create grainy regions and get more attributions on the background or irrelevant objects (\eg the branch and grass highlighted in the 2nd row) than within the objects of interest (\eg the bird).
% Whereas, A-FMI produces smooth and compact regions, which cover the objects of interest well.
% This visually demonstrates that the DeepLIFT and IG suffer from the spread-out pixels, since the pixels are naturally redundant and violate the Relevant characteristic of attribution feature.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{chart/reference.pdf}
%     \vspace{-15px}
%     \caption{\textbf{Reference reliability.} A-FMI is reliable and robust to the different choices of reference. In contrast, both DeepLIFT and IG determine the attribution strongly relative to a chosen reference. B, W, and R stand for black, white, and random reference respectively.} 
%     \vspace{-10px}
%     \label{fig:reference}
% \end{figure}

We observe that DeepLIFT and IG shift their focus when using different references. In particular, the explanations of DeepLIFT and IG with white reference tend to focus on the darker pixels and vice versa. For example, DeepLIFT(W) and IG(W) pay more attention to the black background than the white dog (1st row), while DeepLIFT(B) and IG(B) emphasize the white background surrounding the green apples (2nd row). Moreover, the results of DeepLIFT(R) and IG(R) are unsatisfactory when utilizing a random reference. This verifies that the selection of reference significantly affects the explanations of DeepLIFT and IG.
In contrast, the saliency maps of A-FMI are more consistent, suggesting that the proper reference acts as a prior for A-FMI rather than a hyperparameter.
This validates the robustness and reliability of A-FMI without hinging on instance-by-instance solutions~\citep{input_invariance}. 
% We also observe that, when using different references, the focuses of DeepLIFT and IG are shifted. In particular, the white reference encourages the focus on the darker pixels, and vice versa. For example, DeepLIFT(W) puts more attentions to the black background than the white dog (1st row), while DeepLIFT(B) emphasizes the white background surrounding the green apples rather than the object (3rd row). Moreover, using the random reference makes DeepLIFT(R) and IG(R) unsatisfactory. This verifies that the selection of reference significantly affects the explanations of DeepLIFT and IG.


% \subsection{Class discriminability (RQ3)} \label{sec:class-discriminability}
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{chart/class-specific.pdf}
%     \caption{\textbf{Class discriminability.} A comparison of all methods at a fixed 10\% of important pixels inclusion for different categories. The original image contains exactly two categories -  collie and Ibizan hound. The third category - Cockatoo - is the minimal activated category.}
%     \vspace{-15px}
%     \label{fig:class-specific}
% \end{figure}
% A reasonable prediction explanation is one that produces discriminative visualizations for the class of interest. To measure the class discriminability of attribution methods, a sample image with exactly two categories, a collie and an Ibizan, are conducted to produce visual explanations for both categories as well as the third minimal activated category. The results in Figure~\ref{fig:class-specific} indicate that Gradient, DeepLIFT, IG, and XRAI are unable to achieve class discriminability because the explanation for each class is almost identical for these methods; whereas, class-specific saliency maps can be output by LRP, Grad-CAM, and A-FMI.
% The class prediction mechanism for LRP entails searching for the outline of the object and background (\cf Figure~\ref{fig:introduction}), while Grad-CAM and A-FMI both look for specific traits within the object of interest and expand outward. Moreover, A-FMI produces the most reasonable results because only its result does not contain a portion of the dogs when explaining the minimal activated category.

\subsection{Class Discriminability (RQ3)}\label{sec:class-discriminability}


% A reasonable explanation method should be class discriminable~\cite{Grad-CAM}, which produces different saliency maps for different classes.
% Figure~\ref{fig:class-specific} shows a visual comparison of all methods with a fixed percentage of inclusion on an image with two classes: collie and Ibizan.
% We also display the visual explanation with a minimal activated class: cockatoo.
% Clearly, Gradient, DeepLIFT, and IG hardly generate class-specific explanations, since the pixels highlighted only slightly change after we assign different labels to the attribution methods.
% LRP, Grad-CAM, and A-FMI are able to output class discriminative explanations, which evidently shows that the relationships between explanations and classes are successfully captured.
% Furthermore, we find that LRP is highly likely to outline the edges of objects and background (evidence in Figure~\ref{fig:introduction}), while Grad-CAM and A-FMI get smooth regions.

A reasonable explanation method should be able to produce discriminative visualizations for different class of interest~\citep{Grad-CAM}.
Figure~\ref{fig:class-specific} shows a category-specific visual comparison of all methods with 10\% of insertion on an image with two classes: collie and Ibizan.
We also display the visual explanation with a minimal activated class: cockatoo.
Clearly, Gradient, DeepLIFT, IG, and XRAI hardly generate class-specific explanations, since the significant pixels only slightly change when different labels are assigned.
A-FMI is able to output class discriminative explanations, which evidently shows that the relationships between input and predictions are successfully captured.
Furthermore, we find that LRP is prone to outlining the edges even for background (\cf Figure~\ref{fig:introduction}), while Grad-CAM and A-FMI output tightly identify a region of interest in the image. 

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{chart/class-specific.pdf}
    % \vspace{-5px}
    \caption{\textbf{Class discriminability.} Category-specific visualizations of all methods at a fixed 10\% of important pixels insertion. The original image contains exactly two categories -  Collie and Ibizan hound. The third category - Cockatoo - is the minimal activated category.}
    \vspace{-10px}
    \label{fig:class-specific}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{chart/overall-performance.pdf}
    % \vspace{-5px}
    \caption{\textbf{Visual Inspections.} A visual comparison of all methods, where 5\% and 50\% important pixels are included, respectively. See more examples in Appendix D.
    % Gradient, DeepLIFT and IG tend to produce grainy images, which concentrates on many spurious pixels. LRP, XRAI and Grad-CAM chooses disconnected areas while A-FMI is more refined in the sense that could focus more around the object.
    }
    \vspace{-15px}
    \label{fig:overall-performance}
\end{figure}

% \subsection{Performance comparison (RQ4)}\label{sec:overall-performance}
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{chart/overall-performance.pdf}
%     \caption{\textbf{Overall Performance.} A visual comparison of all methods at 5\% and 50\% important pixels inclusion. Gradient, DeepLIFT and IG tend to produce grainy images, which concentrates on many spurious pixels. LRP, XRAI and Grad-CAM chooses disconnected areas while A-FMI is more refined in the sense that could focus more around the object.}
%     \vspace{-15px}
%     \label{fig:overall-performance}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \subfigure[ACC curves]{
%     \label{fig:acc-zero}\includegraphics[width=0.49\textwidth]{chart/Accuracy-zero.pdf}}
%     \subfigure[ESR curves]{
%     \label{fig:esr-zero}\includegraphics[width=0.49\textwidth]{chart/Explanation-Success-Rate-zero.pdf}}
%     \caption{Accuracy (ACC) curves and Explanation Success Rate (ESR) curves of various attribution methods \wrt different area thresholds. Best viewed in color.}
%     \vspace{-15px}
%     \label{fig:acc-esr}
% \end{figure}

% \begin{table}[t]
% \caption{Explanation performance comparison \wrt area under curves for ACC and ESR.}
% \label{tab:data-statistic}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{c|cccccccc}
% \hline
%  & Random & Gradient & DeepLIFT & IG & LRP & XRAI & Grad-CAM & A-FMI \\ \hline\hline
% ACC-AUC & 0.0493 & 0.1015 & 0.0928 & 0.1409 & 0.3460 & 0.3269 & 0.5324 & $\Mat{0.6187}^{*}$ \\ 
% ESR-AUC & 0.0927 & 0.1708 & 0.1372 & 0.2075 & 0.4194 & 0.4250 & 0.6607 & $\Mat{0.8258}^{*}$ \\ \hline\hline
% Runtime/s & - & - & 0.97 & 5.48 & 5.01 & 22.66 & 6.85 & 1.01 \\ \hline
% \end{tabular}}
% \vspace{-15px}
% \end{table}

% Figure~\ref{fig:overall-performance} shows samples comparison of all methods at 5\% and 50\% important pixels inclusion
% DeepLIFT and LRP tend to initially look for the outline in the image, while the initial important pixels selection for Gradient and IG do not seem to have any discernable pattern. Gradient, DeepLIFT, and IG all become more defined as the threshold increases, however, a large number of pixels are wasted in over-representing unrelated areas, leading to the underestimation of the object of interest. In contrast to other pixel-wise attribution methods, LRP tends to overvalue lines, pixels that run along the edges of the image, and pixels in the corner of the images. 
% XRAI is a non-robust region-level attribution method that sometimes obtains remarkable results, however, sometimes completely incomprehensible. Furthermore, XRAI produces explanations that are discontinuous in nature which will affect its interpretability. 
% Grad-CAM and A-FMI will search for specific characteristics of the object of interest and expand outward. For example, in the case of a dog image, A-FMI will first look for the eyes or nose, then the face, and finally look for the whole body. The results of Grad-CAM tend to become segmented, while the results of A-FMI are more accurate and targeted. Sufficient visual inspections of all methods with thresholds that vary from 5\% to 50\% are provided in the Appendix to differentiate and compare the attribution methods.

% % Sole reliance on visual inspection can sometimes be misleading. Hence, we measure the meaningfulness and quality of pixel-wise attribution scores by sequentially adding pixels from the most important to the least important on a black image. This experiment is conducted on the 279-th Arctic fox class in ImageNet dataset which consists of 1300 images. Two metrics curves for evaluating the performance are considered --- Accuracy (ACC) Curve and Explanation Success Rate (ESR) curve. The x-axis for both curves is the area threshold of pixels adding on a black image, called masked image. For ACC curve (Figure~\ref{fig:acc-zero}), the y-axis is the accuracy calculated over all images for the percentage of important pixels involved. For ESR curve (Figure~\ref{fig:esr-zero}), the y-axis is the proportion of the original label's softmax for the masked image versus the softmax for the original image. If the pixels with the highest attribution scores are identified truly important for the classifier, then the more qualified method should result in the shaper increasing curve. Based on the Figure~\ref{fig:acc-esr} and results of area under curves in Table~\ref{tab:data-statistic}, A-FMI outperforms other attribution methods. 

% Solely relying on visual inspection can sometimes mislead researchers, therefore we elect to evaluate meaningfulness and quality of pixel-wise attribution scores by sequentially adding the most important to least important pixels onto a black image, and monitoring the output of the CNN. This experiment is conducted using the 279th Artic fox class in the ImageNet dataset which consists of 1300 images; wherein two criteria are considered during the evaluation of performance --- Accuracy (ACC) and Explanation Success Rate (ESR) curves. 
% The x-axis is the percentage of pixel inclusion on a black image for both curves, where we call the input image as mask image. For ACC curve (Figure~\ref{fig:acc-zero}), the y-axis is the accuracy calculated across all images for a certain percentage of important pixels inclusion. For ESR curve (Figure~\ref{fig:esr-zero}), the y-axis is the proportion of the original label's softmax for the mask image versus the softmax for the original image. If the pixels with the highest attribution scores are identified truly important for CNN, then a more optimal and efficient method should result in a steeper curve. Based on visual inspection of the curves in Figure~\ref{fig:acc-esr} and a comparison of area under the curve in Table~\ref{tab:data-statistic}, A-FMI outperforms other attribution methods in every metric.

\subsection{Overall Performance Comparison (RQ4)}\label{sec:overall-performance}


\textbf{Visual Inspections}. Figure~\ref{fig:overall-performance} shows that:
1) For pixel-wise attribution methods, at 5\% insertion, DeepLIFT and LRP initially capture outlines, while Gradient and IG fail to find any meaningful patterns.
As the percentage of pixel insertion increases, Gradient, DeepLIFT, and IG become more defined, however, the salient pixels are largely distributed to unrelated areas; meanwhile, LRP tends to overvalue the lines, edges and corners of the images.
2) For region-level attribution methods, XRAI, EP and RISE output more compact regions. However, thier performances are unstable.
3) For feature map-based methods, Grad-CAM and A-FMI tend to initially search for the significant characteristics of target object first (eyes or nose for dog) and then expand outward (body for dog).
Moreover, the explanations of A-FMI are more targeted than Grad-CAM, which suffers from the gradient saturation problem. This verifies the rationality and effectiveness of using references.
Sufficient visualizations of all methods with thresholds that vary from 5\% to 50\% are provided in Appendix D.



% Figure~\ref{fig:overall-performance} shows two samples of all methods with fixed percentage of inclusion (5\% and 50\%). We have the following observations:
% 1) In the line of pixel-wise attribution methods, At 5\% inclusion, DeepLIFT and LRP perform better where the outline gets more attributions, while Gradient and IG hardly find meaningful patterns.
% With the percentage increases, Gradient, DeepLIFT, and IG become more defined, however, the salient pixels are largely distributed to unrelated areas; meanwhile, LRP tends to overvalue lines and pixels along with the edges of any objects.
% 2) As a region-level attribution method, XRAI get more compact regions. However, it has several limitations: first, its performance is unstable and relies heavily on the quality of segments; second, as it is built upon IG, XRAI inherits IG's sensitivity of reference and outputs unsatisfactory explanations when the reference is visually similar to the target objects (see 2nd row).
% 3) In the line of feature map-based methods, Grad-CAM and A-FMI tend to capture the significant characteristics of target classes first (see the face parts in images of dogs) and then expand outward (see the body regions in images of dogs), with the inclusion percentage increases.
% Moreover, the explanations of A-FMI are more targeted than that of Grad-CAM, which might suffer from the gradient saturation problem. This verifies the rationality and effectiveness of using feature map reference.
% More cases are presented in the supplementary material.


\begin{wrapfigure}{r}{0.5\textwidth}
    \vspace{-15pt}
    \begin{center}
        \includegraphics[width=0.235\textwidth]{chart/Accuracy-vgg19.pdf}
        \includegraphics[width=0.235\textwidth]{chart/Accuracy-resnet50.pdf}
    \end{center}
    \vspace{-15pt}
    \caption{Accuracy curves of various attribution methods \wrt different percentage of important pixel insertion (Left: VGG19; Right: ResNet50).}
    \label{fig:acc-esr}
    \vspace{-15pt}
\end{wrapfigure}

\textbf{Predictive Performance}. \emph{Insertion} metric is used to quantitatively evaluate the explanations. \emph{Deletion} metric is not used here since \cite{deletion} has shown its drawbacks.
%Two metrics are used to qualitatively evaluate the explanation.
In particular, we start with a black image, gradually add the pixels with high confidence, and feed this masked image into the CNN model.
As the percentage of pixel insertion increases from 0\% to 100\%, we monitor the changes to classification accuracy (\ie the fraction of masked images that are correctly classified). A sharp increase as well as a higher area under the accuracy curve indicate a better explanation.
In this experiment, we focus on 5000 images sampled from ImageNet and show the results in Figure~\ref{fig:acc-esr} and Table~\ref{tab:auc}\footnote{The results are different from that reported in~\cite{RISE}, where blurred cancaves and probability curve are adopted for insertion.}.
% we focus on the images labeled as ``Arctic Fox'' in the ImageNet training set and show curves of accuracy and softmax ratio in Figure~\ref{fig:acc-esr}, as well as the areas under curves in Table~\ref{tab:auc}.
We find that Grad-CAM and A-FMI consistently outperform the other attribution methods, being able to identify pixels that are truly important to CNN as those with the highest attributions chosen by the methods.
We attribute this success to the Strong Relevance characteristic of feature maps.
Moreover, in VGG19, A-FMI achieves signiﬁcant improvements over Grad-CAM, indicating that using FMI with the reference is a promising solution to the saturation problem; whereas, A-FMI outperforms slightly better than Grad-CAM in ResNet50. This is reasonable since one fully connected layer is involved in ResNet50 and has a minor saturation problem.
% Moreover, in VGG19, A-FMI achieves significant improvements over Grad-CAM, again indicating that combining FMI with the use of references is a promising solution to the saturation problem; in ResNet50, A-FMI consistently outperforms Grad-CAM.
We also find that pixel-wise attribution methods perform relatively poor which is consistent to the visual inspections.
% We also find that LRP is competitive with XRAI, while other pixel-wise attribution methods (Gradient, DeepLIFT, and IG) perform relatively poorly. This observation is consistent with the visual inspections, where LRP and XRAI distribute more attributions around the object of interest.

% We use two evaluation metrics to qualitatively evaluate the explanation quality.
% In particular, we start with a black image, gradually add the pixels with high confidence being significant, and feed this masked image into the CNN model.
% With the percentage of inclusion increases from 0\% to 100\%, We monitor the changes of classification accuracy (\ie the fraction of masked images that are correctly classified) and softmax ratio (\ie the average ratio of the masked image' probability to the original's probability \wrt the class of interest).
% Here we focus on the images labeled as ``Arctic Fox'' in the ImageNet training set, and show the classification accuracy and softmax ratio curves in Figure~\ref{fig:acc-esr}.
% Moreover, the area under each curve is reported in Table~\ref{tab:auc}.
% We find that Grad-CAM and A-FMI consistently outperforms the other attribution methods, revealing the advantages of revealing the most important pixels for the model prediction.
% We attribute this success to the Relevant characteristic of feature maps, which is beneficial to the explanations.
% Moreover, A-FMI achieves significant improvements over Grad-CAM, again indicating that using FMI with the reference is a promising solution to the saturation problem. 
% We also find that LRP is competitive with XRAI, while other pixel-wise attribution methods (DeepLIFT, IG, and Gradient) perform relatively poor. This observation is consistent to the visual inspections, where LRP and XRAI distribute more attributions around regions of interest.





% \begin{figure}[t]
% 	\centering

% % 	\subcaptionbox{Accuracy curves\label{fig:16-soft}}{
% % 		\includegraphics[width=0.235\textwidth]{chart/Softmax Ratio-16.pdf}}
% 	\subcaptionbox{Accuracy \& Softmax Ratio curves on VGG19\label{fig:19-acc}}{
% 		\includegraphics[width=0.235\textwidth]{chart/Accuracy-vgg19.pdf}
% 		\includegraphics[width=0.235\textwidth]{chart/Softmax Ratio-19.pdf}}
% 	\subcaptionbox{Accuracy \& Softmax Ratio curves on ResNet50\label{fig:16-acc}}{
% 		\includegraphics[width=0.235\textwidth]{chart/Accuracy-resnet50.pdf}
% 		\includegraphics[width=0.235\textwidth]{chart/Softmax Ratio-16.pdf}}
% % 	\subcaptionbox{Softmax ratio curves\label{fig:19-soft}}{
% % 		\includegraphics[width=0.235\textwidth]{chart/Softmax Ratio-19.pdf}}
% 	\vspace{-5pt}
% 	\caption{\textbf{Predictive Performance I}. Accuracy curves and Softmax ratio curves of various attribution methods \wrt different percentage of important pixels inclusion. Best viewed in color.}
% 	\label{fig:acc-esr}
% 	\vspace{-15pt}
% \end{figure}

\begin{table}[t]
    \caption{Performance comparison \wrt area under curves of Accuracy.}
    \label{tab:auc}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l|ccccccccccc}
    \hline
    Accuracy-AUC & Random & Gradient & DeepLIFT & IG & LRP & XRAI & EP & RISE & GradCAM & \textbf{A-FMI} \\ \hline\hline
    VGG19 & 0.0854 & 0.1657 & 0.1673 & 0.2177 & 0.3460 & 0.3269 & 0.1775 & 0.2596 &  0.5343 & $\mathbf{0.5908}^{*}$ \\ 
    ResNet50 & 0.0854 & 0.2236 & 0.1812 & 0.2857 & - & - & 0.2613 & 0.2970 &  0.6380 & $\mathbf{0.6513}^{*}$ \\ \hline\hline
    Time per image/s & - & 0.0354 & 0.0669 & 1.5908 & 0.9719 & 14.6469 & 14.1818 & 10.8123 & 0.0291 & 0.1392 \\ \hline
    \end{tabular}}
    \vspace{-10px}
\end{table}


% \begin{table}[h]
% \caption{Performance comparison \wrt area under curves of Accuracy and Softmax Ratio.}
% \label{tab:auc}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
% \hline
%  &  & Random & Gradient & DeepLIFT & IG & LRP & XRAI & Grad-CAM & A-FMI \\ \hline\hline
% \multirow{2}{*}{VGG19} & Accuracy-AUC & 0.0493 & 0.1015 & 0.0928 & 0.1409 & 0.3460 & 0.3269 & 0.5324 & $\Mat{0.6187}^{*}$ \\ %\cline{2-10} 
%  & Softmax-AUC & 0.0927 & 0.1708 & 0.1372 & 0.2075 & 0.4194 & 0.4250 & 0.6607 & $\Mat{0.8258}^{*}$ \\ \hline\hline
% \multirow{2}{*}{VGG16} & Accuracy-AUC & 0.0771 & 0.1676 & 0.1719 & 0.1507 & 0.2208 & 0.3885 & 0.5753 & $\Mat{0.6559}^{*}$ \\ %\cline{2-10} 
%  & Softmax-AUC & 0.2510 & 0.3419 & 0.3632 & 0.3587 & 0.5390 & 0.7255 & 0.7895 & $\Mat{0.8413}^{*}$ \\ \hline\hline
% \multicolumn{2}{|c|}{Compute Time per image/s} & - & 0.0354 & 0.0669 & 1.5908 & 0.9719 & 14.6469 & 0.0291 & 0.1392 \\ \hline
% \end{tabular}}
% \vspace{-15px}
% \end{table}

% \begin{table}[t]
% \caption{Explanation performance comparison \wrt area under curves for ACC and ESR.}
% \label{tab:auc}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{c|cccccccc}
% \hline
%  & Random & Gradient & DeepLIFT & IG & LRP & XRAI & Grad-CAM & A-FMI \\ \hline\hline
% ACC-AUC & 0.0493 & 0.1015 & 0.0928 & 0.1409 & 0.3460 & 0.3269 & 0.5324 & $\Mat{0.6187}^{*}$ \\ 
% SOFT-AUC & 0.0927 & 0.1708 & 0.1372 & 0.2075 & 0.4194 & 0.4250 & 0.6607 & $\Mat{0.8258}^{*}$ \\ \hline\hline
% Compute time/s & - & 0.0354 & 0.0669 & 1.5908 & 0.9719 & 14.6469 & 0.0291 & 0.1392 \\ \hline
% \end{tabular}}
% \vspace{-15px}
% \end{table}

% \begin{figure}[t]
% 	\centering
% 	\subcaptionbox{Accuracy curves\label{fig:acc-zero}}{
% 		\includegraphics[width=0.49\textwidth]{chart/Classification Accuracy-zero.pdf}}
% 	\subcaptionbox{Softmax ratio curves\label{fig:esr-zero}}{
% 		\includegraphics[width=0.49\textwidth]{chart/Softmax Ratio-zero.pdf}}
% 	% \vspace{-15pt}
% 	\caption{Accuracy curves and Softmax ratio curves of various attribution methods \wrt different percentage of important pixels inclusion. Best viewed in color.}
% 	\label{fig:acc-esr}
% 	\vspace{-15pt}
% \end{figure}



\textbf{Computational Performance}.
In terms of time complexity, we report the time cost per image of each attribution method and find that, A-FMI performs similarly to the pixel-wise attribution methods while being significantly faster than the region-level attribution methods.

==> Arxiv2021_ A-FMI/5_conclusion.tex <==
\section{Conclusion}
We proposed a novel attribution method via feature map importance, A-FMI, to produce visual explanations for CNNs.
A-FMI provides a potential way to solve the gradient saturation problem at the granularity of feature maps, which allows the information to be backpropagated even when the gradient approaches zero.
Extensive experiments illustrated the superior performance of A-FMI from both interpretable and faithful perspectives, compared with other popular attribution methods.
Future work includes
% we plan to produce high-resolution saliency maps that A-FMI failed to do, in order to get finer-grained explanations.Furthermore, 
applying the attribution methods to other types of neural networks, such as graph neural networks.




% Although our visualizations outperformed most existing attribution methods from both interpretable and faithful perspectives, we believed that pixel-wise attribution methods remain valuable to gain high-resolution saliency map that A-FMI failed to do. Future works include how to apply A-FMI to deep networks such as reinforcement learning and how to obtain fine-grained details explanation by A-FMI.    

%We believe an important research agenda is furthering .... that guarantee reliability ....
%This work is motivated by our belief that pixel-wise saliency methods remain valuable approaches to gain intuition about the network. Understanding where they fail equips researchers with the tools to appropriately weigh the explanations these models provide.

%Determining how saliency methods fail is an important stepping stone to understanding where and how we should use these methods. An urgent research agenda, and a requirement for the use of deep neural networks in domains like medicine, is evaluating which methods and/or reference points consistently guarantee reliability for all possible transformations.

==> Arxiv2021_ A-FMI/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

